LatentDR: Improving Model Generalization Through Sample-Aware Latent Degradation and Restoration

Despite significant advances in deep learning, models often struggle to generalize well to new, unseen domains, especially when training data is limited. To address this challenge, we propose a novel approach for distribution-aware latent augmentation that leverages the relationships across samples to guide the augmentation procedure. Our approach first degrades the samples stochastically in the latent space, mapping them to augmented labels, and then restores the samples from their corrupted versions during training. This process confuses the classifier in the degradation step and restores the overall class distribution of the original samples, promoting diverse intra-class/cross-domain variability. We extensively evaluate our approach on a diverse set of datasets and tasks, including domain generalization benchmarks and medical imaging datasets with strong domain shift, where we show our approach achieves significant improvements over existing methods for latent space augmentation. We further show that our method can be flexibly adapted to long-tail recognition tasks, demonstrating its versatility in building more generalizable models. Code is available at https://github.com/nerdslab/LatentDR.

==> tables/DomainNet_breakdown.tex <==
\begin{table}[t]
\caption{Classification accuracies on DomainNet.}
\label{table:pacs}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccccr}
\hline
Model & 0 & 1 & 2 & 3 & 4 & 5 & All \\
\hline\hline
OURS (1) & 62.5 & 21.7 & 51.1 & 13.3 &  \\
% might need to run DomainNet w SGD instead of Adam
OURS (2) &  &  &  &  &  \\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/OH_breakdown.tex <==
\begin{table}[t]
\caption{Classification accuracies on OH.}
\label{table:pacs}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccr}
\hline
Model & 0 & 1 & 2 & 3 & All \\
\hline\hline
OURS (1) & 65.9 & 56.0 & 77.3 & 79.4 & 69.7 \\
OURS (2) & 62.1 & 53.3 & 75.6 & 77.3 & 67.1 \\
OURS (3) & 65.3 & 54.9 & 77.3 & 78.5 & 69.0 \\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/PACS_breakdown.tex <==
\begin{table}[t]
\caption{Classification accuracies on PACS. Following domain generalization protocols, the encoder architecture is a ResNet-18 that is pre-trained on ImageNet. The superscript $^{c}$ means the numbers are copied from their paper. Numbers from MixStyle and BatchFormer.}
\label{table:pacs}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccr}
\hline
Model & A & C & P & S & All \\
\hline\hline
%ERM  & 79.6 & 72.7 & 95.4 & 77.0 & 81.2 \\
%Mixup$^{c}$ & 76.8 & 74.9 & 95.8 & 66.6 & 78.5 \\
%Manifold Mixup$^{c}$ & 75.6 & 70.1 & 93.5 & 65.4 & 76.2 \\
%MixStyle$^{c}$ (random) & 82.3 & 79.0 & 96.3 & 73.8 & 82.8 \\
%MixStyle$^{c}$ (cross) & 84.1 & 78.8 & 96.1 & 75.9 & 83.7  \\
%BatchFormer$^{c}$ & 80.4 & 73.8 & 96.3 & 68.6 & 79.8 \\
OURS (1), ResNet50 & 87.5 & 80.6 & 97.7 & 75.4 & 85.3 \\
OURS (2) & 88.4 & 79.5 & 97.5 & 78.2 & 85.9 \\
OURS (3) & 87.4 & 81.2 & 97.8 & 76.7 & 85.8 \\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/Terra_breakdown.tex <==
\begin{table}[t]
\caption{Classification accuracies on TerraIncognita. Following domain generalization protocols, the encoder architecture is a ResNet-50 that is pre-trained on ImageNet. The superscript $^{c}$ means the numbers are copied from their paper.}
\label{table:pacs}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccr}
\hline
Model & L100 & L38 & L43 & L46 & All \\
\hline\hline
ERM  & 50.2 & 34.9 & 55.2 & 32.1 & 43.1 \\
Mixup & 60.5 & 43.7 & 56.5 & 22.9 & 45.9 \\
Manifold Mixup & & & & & \\
CORAL & 52.4 & 43.2 & 55.4 & 36.9 & 47.0 \\
MixStyle & & & & & \\
BatchFormer & 47.3 & 43.8 & 54.5 & 38.9 & 46.1 \\
OURS (1) & 49.1 & 41.5 & 59.2 & 41.2 & 47.8 \\
OURS (2) & 51.4 & 43.1 & 57.3 & 40.7 & 48.1 \\
OURS (3) & 49.6 & 47.1 & 58.2 & 44.2 & 49.8 \\



% OURS (2) & 52.4 & 39.8 & 59.5 & 41.1 & \textbf{48.2} \\
% OURS (3)
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/VLCS_breakdown.tex <==
\begin{table}[t]
\caption{Classification accuracies on VLCS.}
\label{table:pacs}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccr}
\hline
Model & 0 & 1 & 2 & 3 & All \\
\hline\hline
OURS (1) & 98.1 & 65.4 & 74.3 & 77.3 & 78.8 \\
OURS (2) & 97.7 & 65.1 & 76.6 & 77.3 & 79.2 \\
OURS (3) & 97.8 & 64.5 & 73.9 & 78.4 & 78.7 \\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> texts/ablations.tex <==
\vspace{-2mm}
\subsubsection{Ablations and visualizations}
\vspace{-2mm}
To further understand the robustness of the proposed method, we perform model ablation, latent representation evaluation, and nearest neighbor visualization
% and study the latent representations obtained 
with our model on the PACS dataset.

\vspace{-3mm}
\paragraph{The effect of latent degradation.}~
\label{para:degrade}
We first investigate the effect of sample-aware latent degradation by decomposing the degradation and restoration steps as in Table \ref{table-ablation}. Specifically, we test adding only the degradation loss (D-only) under two settings: (1) Sample-aware degradation (\ours) and (2) additive Gaussian noise (Gaussian).
% and adding only the restoration loss (R-only). 
When no restoration is present, we show that awareness of sample distribution is critical,
%latent degradation step is critical to our method, 
%as the model performs better when no restoration is present, 
as our sample-aware latent degradation might be an effective augmentation operation by itself that improves model performance in contrast to performance dropping with additive Gaussian noise. A similar effect is observed in \cite{li2021simple}.
% Without latent degradation, our method boils down to \cite{hou2022batchformer}, where the performance does not systematically improve in many benchmarks. Combining the sample-aware latent degradation with latent restoration, our method D+R achieves the best performance.

To understand whether the degradation is indeed producing outputs that confuse the classifier, we examined the classification accuracy for the degraded latents and obtained an average accuracy of $33\%$ for a 7-way classification (random guess rate is $14\%$). 
% We conjecture that it is possible that this classifier-guidance may encourage certain content/style separation in the latent space.

\begin{table}[t]
\begin{center}
% \begin{small}
% \begin{sc}
\begin{tabular}{lcccccr}
%\hline
&  & P & A & C & S & Avg. \\
\hline
Reference & ERM & 84.9 & 80.6 & 95.9 & 75.0 & 84.1 \\
\hline
\multirow{3}{*}{Ours} 
& D-only & 85.7 & 78.6 & 96.9 & 78.2 & \underline{84.8} \\
& R-only & 82.6 & 79.3 & 95.4 & 73.5 & 82.7 \\
& D+R & 86.3 & 82.6 & 97.1 & 79.2 & \textbf{86.3} \\
\hline
\multirow{3}{*}{Gaussian} 
& D-only & 85.0 & 78.1 & 96.5 & 75.6 & 83.8 \\
& R-only & 86.4 & 80.0 & 97.4 & 76.5 & \underline{85.1} \\
& D+R & 87.4 & 79.7 & 97.1 & 77.1 & \textbf{85.3} \\
\hline
\end{tabular}
% \vskip 0.15in
% \end{sc}
% \end{small}
\end{center}
\caption{\textit{Ablations of degradation and restoration on PACS}. We compare the performance of \ours~using the degradation loss (D-only) or restoration loss (R-only) alone vs. combining them (D+R), for our sample-aware degradation approach (top) vs. additive Gaussian noise (below).}
\label{table-ablation}
\vspace{-3mm}
% \vskip -0.1in
\end{table}

\vspace{-3mm}
% \paragraph{Decomposing the degradation and restoration steps.}
\paragraph{The effect of latent restoration.}
We next test if latent restoration can improve performance by itself. Without any latent degradation, our method boils down to \cite{hou2022batchformer}, which does not systematically improve performance in many benchmarks. However, when replacing sample-aware latent degradation with additive Gaussian noise, latent restoration (Gaussian R-only) outperforms the ERM baseline, indicating that our restoration procedure could be effective when combined with other forms of  degradation.

%We next tested the effect of degrading latents in our model using Gaussian noise with (Gaussian D-R)  and without restoration (Gaussian D-only). In the case where we do not restore the latents, we see a marked decrease in overall performance. In contrast, when we restore the latents after a Gaussian noise perturbation, we see that the model can still benefit over the ERM baseline. However, 
Combining both sample-aware degradation  with  restoration, we obtain the best overall performance (D+R).
On the other hand, with additive Gaussian noise, combining degradation and restoration steps (Gaussian D+R) does not show performance improvements when compared to using restoration only (Gaussian R-only).
%while Guassian D+R does not further improve the performance in comparison to Guassian R-only.
This suggests that our proposed latent degradation and restoration procedures work in tandem, and it is critical to consider sample-to-sample relationships to have the most impact on out-of-domain generalization. 
% The similar effect is shown in \cite{li2021simple}.

%\vspace{-3mm}
%\paragraph{The effect of latent restoration under Gaussian noise.}
%How would latent restoration take effect when the degradation step is guided by Gaussian noise?
%To answer this question, we replace the degradation process with Gaussian noise and add the restoration loss to regularize the learning. As shown in Table~\ref{table-ablation} (Gaussian R-only), latent restoration provides performance boost even when the degradation is guided by Gaussian noise, although the degradation step is not helping (Gaussian D+R).
%This suggests that our approach could admit many variants and it can be possible to replace the latent degradation part with a simpler format of noise (e.g. Gaussian noise) in certain cases.

\begin{figure*}[t!]
\begin{center}
 \includegraphics[width=\textwidth]{images/latent_viz-07.png}
 \end{center}
\vspace{-2mm}
\caption{
\small {\em Nearest neighbors visualizations.} We show the top two nearest neighbors for a query sample after degradation (top row) and restoration (bottom row). In the leftmost example, we find a case where degradation places a sample near points from a different class but brings it back to diverse domains from its original class. On the right, we show examples where degradation maps the latent next to samples of the same class that are different in color or background, and restores to samples that are similar but might be from another domain. 
%Latent restoration transports samples into different parts of the latent space
\label{fig:neighbors}}
\vspace{-4mm}
\end{figure*}


 \begin{figure}[t!]
\begin{center}
 \includegraphics[width=0.46\textwidth]{images/uni_aln_ran.png}
 \end{center}
   \caption{\textit{Latent quality evaluation.} We measure the uniformity and alignment of the latent spaces for ERM, Mixup \cite{zhang2017mixup}, BatchFormer \cite{hou2022batchformer} (BF), and \ours~(Ours-SA).\vspace{-2mm}}
 \label{fig:latents-metrics}
 \vspace{-2mm}
\end{figure}


%\vspace{-3mm}
%\paragraph{Sharing classifier weights.}
% Our model trains a classifier $g$ on top of the encoder $f$, and uses the same classifier $g$ to regularize the model to learn degraded samples and restored samples. Following \cite{hou2022batchformer}, we tested whether training two different classifiers, one for the original loss, and the other for the corruption/restoration steps, would benefit the training. With a separate classifier, our model gets an average of $83.7\%$ accuracy on PACS, an over 2\% decrease. It seems it is critical to share classifier weights for our method.
% , different from \cite{hou2022batchformer}.


\vspace{-3mm}
% \paragraph{Examining the latents and the effect of restoration.} 
\paragraph{Latent quality evaluation.} 
To understand how the model is shaping the representations of the data, we examined the uniformity and alignment metrics for different models as shown in Figure~\ref{fig:latents-metrics} (see Appendix~\ref{appendix:latents} for direct visualizations). We confirmed that our method not only gives the highest uniformity score, which demonstrates that it preserves the maximum amount of information inside the training data  but also gives the lowest alignment score, which demonstrates that it encourages the closeness of latents within the same class. Interestingly, we find that Mixup \cite{zhang2017mixup} does improve alignment but has very little improvement in uniformity when compared with ERM. On the other hand, BatchFormer \cite{hou2022batchformer} produces good diversity of latents by considering nonconvex sample-to-sample relationships but poorer alignment. Our method, instead, combines the advantages at both ends by encouraging the diversity of the generated samples while maintaining good alignment by separating the different classes.

\vspace{-3mm}
\paragraph{Nearest neighbor visualization.} 
To observe how the degradation and restoration steps remap different query points, we examined the nearest neighbors of the augmented latents for both operations (Figure~\ref{fig:neighbors}). We observed that indeed the latents produced from the latent restoration process would retrieve nearest neighbors to samples from the same class but different domains (both the testing domain and another training domain).
% near samples that are from the same class, but often the new nearby point is from a different domain (both the testing domain and another training domain). 
Interestingly, in the degradation step, although the produced samples would often confuse the classifier, the nearest neighbors are often from the same class but with dissimilar colors or backgrounds.
% the class may be switched but more often than not when the model is fully trained, although the nearest neighbors typically would match samples with different colors or backgrounds.
We conjecture that it is possible that this classifier guidance may encourage certain content/style separation in the latent space.


==> texts/additional_backbone.tex <==
\paragraph{Using another backbone.}
As discussed in \cite{cha2022domain}, when testing on domain generalization applications, it is not necessarily better to use larger-scale backbone models, as naively fine-tuning the pre-trained models on DG might worsen the performance. 
To validate the effectiveness of our method when using a larger-scale backbone, we selected ViT-B which is pre-trained on ImageNet-21k and benchmarked a few methods on top.
We show that our data augmentation operation is robust when testing with a larger-scale backbone, which demonstrates its potential when applied together with other models.

Performance on OfficeHome improves a lot for all the methods. But we are able to get a very strong performance as compared to others. A potential reason could be the difficulty of the OfficeHome dataset. PACS and VLCS have 7 and 5 classes each, but OfficeHome has 65 classes. And the three datasets have similar number of datapoints (9991, 10729, and 15588 respectively). Due to this, OfficeHome has a lot of room for improvement, hence a stronger backbone that is pre-trained on ImageNet-21k seems to utilize this potential and we are able to notice significant improvements in performance on this dataset.


\begin{table}[h!]
\caption{Results with a ViT backbone pre-trained on Imagenet.}
\vskip 0.15in
\begin{center}
%\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\hline
& PACS & VLCS & OfficeHome & Avg. \\
\hline
CORAL & 85.9 & 75.3 & 75.3 & 78.8 \\
% MIRO &  &  &  & \\
ViT-B & 82.6 & 77.8 & 75.6 & 78.7 \\
+ Mixup & 84.8 & 76.9 & 75.7 & 79.1 \\
+ BF & 80.2 & 76.8 & 75.0 & 77.3 \\
\hline
+ Ours (SA) & 84.5 & 79.0 & 77.1 & 80.2 \\
+ Ours (Pool) & 86.4 & 78.6 & 77.3 & 80.8 \\
\hline
\end{tabular}
% \end{sc}
%\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> texts/additional_explain.tex <==
\subsubsection{Intuitive explanation of latent degradation}

We provide more intuitive explanations of our latent degradation operation from the perspective of the Vicinal Risk Minimization (VRM) principle. 
% While the following contents aim to provide 
% , hoping to provide future research opportunities.
% \paragraph{Vicinal Risk Minimization (VRM).}
% below rewrote from Mixup
% below rewrote from Mixup
% below rewrote from Mixup
% need further edit (simplify)

The goal of supervised learning is to learn a function $f(\cdot)$ that studies the relationship between data $X$ and target $Y$, which follows the joint distribution $P(X, Y)$. Specifically, consider a loss function $\ell$, the goal is to minimize the expected risk:
\[
R(f)=\int \ell(f(x), y) \mathrm{d} P(x, y)
\]
where the goal is to minimize the expected loss over the data distribution $P$.

Unfortunately, the distribution $P$, in practice, is limited by the diversity of the training data. $(\mathcal{X}, \mathcal{Y})=\left\{\left(x_i, y_i\right)\right\}_{i=1}^n$, where $\left(x_i, y_i\right) \sim P$ for all $i$. The empirical distribution $P$ by the empirical distribution is approximated using the training data:
\[
P(x, y)=\frac{1}{n} \sum_{i=1}^n \delta\left(x=x_i, y=y_i\right),
\]
where $\delta\left(x=x_i, y=y_i\right)$ is a Dirac mass centered at $\left(x_i, y_i\right)$. 

What Mixup did is that:
\begin{gather*}
    %\begin{array}{r}
    \tilde{x}=\lambda x_i+(1-\lambda) x_j \\
    \tilde{y}=\lambda y_i+(1-\lambda) y_j \\
    %\end{array} \\
    \mu\left(\tilde{x}, \tilde{y} \mid x_i, y_i\right)=\frac{1}{n} \sum_j^n \underset{\lambda}{\mathbb{E}}\left[\delta\left(\tilde{x}, \tilde{y}\right)\right]
\end{gather*}
which replaces the original distribution such that:
\[
P_\nu(\tilde{x}, \tilde{y})=\frac{1}{n} \sum_{i=1}^n \nu\left(\tilde{x}, \tilde{y} \mid x_i, y_i\right)
\]
However, in reality, Mixup often selects $\alpha$ from a Beta distribution, which is often close to its original point, and provide limited diversity.

From this perspective, our degraded operator can be viewed as creating a non-convex version of Mixup.

% \paragraph{Content/style separation.}
% \paragraph{Preventing trivial solution.}

BatchFormer could obtain a trivial solution in the sense that the Transformer might just return an Identity matrix, although it has a high dropout rate. Our joint latent augmentation and label augmentation, instead, would prevent the trivial solution. Thus, it works even better, when combined with the restoration operator.


==> texts/intro_Feb16.tex <==


Although deep neural networks have demonstrated robust performance learning representations, the generalizability of deep neural networks are often achieved because of the diversity of the training data, which is challenging or infeasible in many real-world applications. Domain generalization (DG) aims to address this issue by learning robust representation of data by training only on source domains, but testing on unseen domain without prior training or domain assumptions. The scarcity of available training data made DG a very challenging problem.

One approach that has been widely used to improve generalization is to augment training examples, often through corrupting and masking training samples. For instance, image masking and cutout are based on masking the majority of the data, and mixup is a widely used approach to build new virtual samples as a combination of two existing samples from the training set, which is theoretically shown to be related to adversarial learning \cite{zhang2020does}. However, the nature of convex combination as data augmentation operations does not build enough connections across domains, where style statistics are separated during learning (demonstrated by Mixstyle \cite{zhou2021domain}). Existing works trying to generate new domain \cite{zhou2020learning} are very complex. How to perform data augmentations that build connections across domain and diversity domain information to improve generalization is an open question.

\begin{figure}[t]
\centering
  \includegraphics[width=0.45\textwidth]{images/overview_dg_pool.png}
  \caption{Overview of the high-level idea of the model. We can either use a real latent space figure, or a toy figure like this.}
\end{figure}

In this work, we explore how the idea of both corruption and restoration can be directly applied on latent space to build robustness against domain shift. Our work takes some inspiration from diffusion models where the aim is to both learn a forward and inverse process to add noise and recover the signal again. 
Specifically, we train two transformers, one that transforms the latents across a batch to make them indiscernible by a classifier, and the other to restore the noisy latents through a cross-attention transformer \cite{jaegle2021perceiver,rombach2022high}.
Similar as \cite{hou2022batchformer}, our approach is flexible and pluggable in mini-batch training, and builds sample-to-sample relationship into the model training process, which can be applied to a wide range of architectures and problem settings. 
% Because latent restoration is applied during training and removed during testing, we can view it as a robust data augmentation operation.

We systematically evaluated our method on standard domain generalization benchmarks (DomainBed \cite{gulrajani2020search}) using the standard evaluation protocal, and then apply the method to a diverse set of medical imaging datasets where batch effects and domain shift occurs. Finally, we provide experiments which highlight the application of the method on long-tail recognition tasks. 
To further quantify the improvements, and to further investigate and understand why the proposed method is effective, we used uniformity and alignment \cite{wang2020understanding} to understand the latent quality, and used nearest neighbor visualization to understand how the data augmentation is taking effect. Our model shows that our batch-level augmentation procedure not only improves the overall quality of latents along both metrics, and the augmentation process was producing extrapolation and interpolation of samples that effectively build connections across domains.

To conclude, our work has the below contributions:
(1) We explored the possibility of using the process of latent restoration as an effective data augmentation operation on images, assisting a normal backbone model. This is the first work that conceptually do this
\colortext{Need to check if this claim is accurate};
(2) We combine the sample-to-sample relationship research with a classifier-guided restoration process, which created a pluggable and removable part of the model, that is parameter-free during inference;
(3) We demonstrated the robustness of our method on domain generalization tasks, which opened up a lot of possibilities for the proposed method;
(4) We applied a set of visualization and metrics to understand the method.



==> texts/intro_eva.tex <==

\section{Introduction}
In machine learning, it is often challenging to train a model that generalizes well when tested on domains that it was not exposed to during training \cite{ben2010theory}. This is especially true when the available training data is limited, %\zkn{One thought, which maybe can be done for supplementary, is that your main experiment (domainnet) is not data-limited. If you want to drive this point, might be nice to do low-labeled version (where you sub-sample labeled data) and do this new setting. You'd also do this for a few top DG methods}, 
 as is often the case in real-world applications. Various methods have been proposed to address this challenge, including feature alignment approaches \cite{sun2016deep,ganin2016domain}, meta-learning \cite{sankaranarayanan2023meta,balaji2018metareg}, and data augmentations \cite{volpi2018generalizing,zhou2020deep}. However, achieving robust out-of-domain (OOD) generalization remains a challenging problem \cite{gulrajani2020search}, and further research is needed to develop more effective methods.

\begin{figure}[t!]
\centering
  \includegraphics[width=0.45\textwidth]{images/Fig1_ran_edit2.png}
  \caption{\small {\em Visualization of latent degradation and restoration steps during training.} In \textbf{(A)}, when it is earlier in training, latents from different domains are separated for the same class, which hurts model generalization. To tackle this issue, for each {latent query} ({\color{red}{$\star$}}), \ours~first {degrades} ({\color{blue}{$\times$}}) them to a point that is far away from the existing domains, and {restores} ({\color{darkergreen}{$\blacktriangledown$}}) them back to the existing distribution to diversify existing domains and improve model generalization. In \textbf{(B)}, 
  % In (A), we visualize the latent space for a single class early in training when samples from different domains are separated\zk{Is this a good or bad thing?}. 
  % For a single query point (red star), we simulate different possible augmentations generated by our model (blue x's) and their restored versions (green triangle). 
  % In (B), 
  we visualize the latents for all classes at a later point in training and color data by classes.\label{fig:fig1}\vspace{-3mm}}
  % \zk{Great figure! Number ``(1) Degrade'' ``(2) Restore'' in the figure. Also, ``all class'' to ``all classes''}\label{fig:fig1}\vspace{-3mm}}
\end{figure}

% In the field of domain generalization, one emerging technique for addressing the challenges of heterogeneous training data is {\em latent augmentation}. 
Among existing strategies, one emerging technique for addressing the problem of OOD~generalization is {\em latent augmentation}.
Similar to data augmentation methods, the overall objective of latent augmentation is to increase the diversity of the source data so that the model is encouraged to learn domain-agnostic representations \cite{verma2019manifold}. However, different from data augmentation methods which directly manipulate the data space, 
% through data transformations or novel examples generation, 
latent augmentation modifies the hidden data representations or feature space of a model, which avoids the usage of generative networks \cite{zhou2020deep}, additional classifiers \cite{shankar2018generalizing}, or adversarial training \cite{volpi2018generalizing}.
% In contrast, latent augmentation modifies the hidden data representations or feature space of a model to directly enhance its ability to handle domain shifts. 
Many existing latent augmentation methods typically assume that linear combinations \cite{verma2019manifold}, the mixture of style statistics \cite{hong2021stylemix,somavarapu2020frustratingly}, or additional randomization \cite{li2021simple} of hidden representations can provide the desired diversity for generalization. However,
when dealing with highly diverse domains, using simple assumptions (like linear mixing) is often insufficient \cite{cha2021swad}, and generating robust latent augmentations remains an outstanding challenge.

%Therefore, we must explore more robust methods for latent augmentation, capable of generating diverse latents beyond those simple assumptions.

% The simplicity of assumptions has limited the performance boost when facing highly heterogeneous domains. Moving forward, we need more robust latent augmentation methods that could generate diverse latents let along those assumptions.

% these methods may not be effective when the training data is highly heterogeneous, and generating good latent augmentations remains an outstanding challenge.

% As a result, latent augmentation offers a promising approach to improve the robustness of machine learning

% While data augmentation approaches have demonstrated robustness towards domain shifting  by increasing the diversity of the source data through either domain-agnostic transformations or generating adversarial examples, they require the operations to be performed in the data space directly, which requires the training of generative networks, additional classifiers, or adversarial training pipelines. On the other hand,
% latent augmentation focuses on modifying the hidden data representations or feature space of a model to increase its robustness to domain shifts \cite{yosinski2014transferable,verma2019manifold}.
%By learning to identify and manipulate the relevant latent factors that vary across domains, a model can better adapt to new unseen domains with reduced overfitting to training domains. 
%without overfitting to any single domain.

% In this paper, we propose \ours,\zkn{What does DR stand for?} a novel latent augmentation approach for improving domain generalization. To build our latent augmentation approach, we take inspiration from diffusion models \cite{ho2020denoising,rombach2022high}. 

%Addressing limitations of simple sample-to-sample mixing in prior works, we leverage batch-level sample-to-sample mixing through self-attention to perform this degradation/restoration, 3) Crucially, the restoration process is conditioned on the non-corrupted latents, using sample-to-sample relationships including to non-corrupted latents. 

%Here, we propose a novel approach that aimsproduces latent augmentation


Here, we propose a novel latent augmentation approach for improving  generalization called \ours. We take inspiration from diffusion models that generate diverse but realistic samples \cite{ho2020denoising,rombach2022high}:
% that combines Latent Degrade and Restore
In both our model and in diffusion, the goal is to not only {\em degrade} samples but also to {\em restore} them back to their original state.
To learn to degrade and restore latents, we leverage attention to incorporate information from other samples in the batch during training.
% sample-to-sample\zkn{How? Through what mechanism? Include more specific descriptions e.g. from line 216 in related work} relationships across the latent distribution during training. 
The idea is shown in Figure~\ref{fig:fig1}(A): The degradation process aims to map the query to a point where its class cannot be easily distinguished by a downstream classifier; 
%where we construct corresponding soft labels to help the network to learn a more robust decision boundary.
% and thus the degraded samples can be used to create a more robust decision boundary.
the 
% In the degradation stage, the aim is to map the query to a point where its class cannot be distinguished; 
% In the 
restoration process uses the %permutation-invariant 
cross-attention mechanism \cite{vaswani2017attention,jaegle2021perceiver} to 
(only) recover the class information from the degraded latents by conditioning on the original latents. 
By combining degradation and restoration, \ours~encourages the model to capture the relationship across samples from different classes and domains, and thus guides the model to generalize better to unseen sources.
% through sample-aware latent augmentation.
%provides restored samples 
% with perturbed domain information 
%that can be used to diversify the training samples in the latent space.
% condition the degraded latents on the original latents.\zkn{Describe the motivation for cross-attention to condition on original latents; explicitly describe: what does this achieve and how?} 
% and uses degraded latents as queries. 
% During this process, the augmented sample should retain its critical semantic meaning while also generating diverse samples.
% By doing this, \ours~not only uses degraded samples to create a more robust decision boundary, but also uses restored samples to diversify the training samples in the latent space\zkn{Tie directly to cross-attention}.
% build better connections across domains by generating diverse samples.
% We show that by combining  degradation and restoration, \ours~can guide the model to learn representations that generalize better to unseen domains.


To demonstrate the utility of our approach in diverse settings, we conduct experiments on: (i) five standardized domain generalization benchmarks \cite{gulrajani2020search,cha2021swad},
(ii) five medical imaging classification datasets that suffer from 
domain shifting issues \cite{koh2021wilds,yang2023medmnist}, and (iii) 
% to show the generality of our approach to other settings, 
a long-tail (LT) recognition task where 
our latent augmentation technique can improve generalization in the presence of strong data imbalance.
% across imbalanced data.
% class imbalance is present and data augmentation can be used to ameliorate the effects of this  \cite{hou2022batchformer}
% \zkn{This still comes out of nowhere. I added something to justify but could use some rewording maybe}
In all of these cases, we provide impressive boosts over other augmentation-based approaches on all of the datasets tested, and competitive performance with state-of-the-art methods that use more complex losses and domain information. To better understand the effectiveness of our approach on learning, we use two measures of representation quality \cite{wang2020understanding} and nearest neighbor visualization to measure the impact of our approach.


% To further quantify the impact that our approach has on learning, we use two measures of representation quality \cite{wang2020understanding} and nearest neighbor visualization to understand how the latent augmentation is taking effect.


% \paragraph{Contributions.} 
% In summary, the contributions of our work include: \textbf{(i)} We propose a novel approach for latent augmentation that aims to build connections across samples from different domains by both \textit{degrading} and \textit{restoring} the samples from the latent distribution. We utilize sample-to-sample relationships in both the degradation and restoration processes, and use classifier guidance to encourage the mixing of samples across domains.
% \textbf{(ii)} We conduct empirical studies to demonstrate that our approach improves class-level alignment of features, as well as the uniformity or spread of the data distribution. These two metrics have been shown to be useful for pre-training models for different downstream tasks.
% \textbf{(iii)} We evaluate the robustness of our method on domain generalization benchmarks and medical imaging datasets with domain shift. We also provide various ablations to better understand the method. Finally, we demonstrate the versatility of our method by testing it on a long-tail recognition task.

%\zkn{This bullet list has a lot of whitespace. Not sure if it's non-conformant, but there are arguments to itemize that can reduce this}
In summary, the contributions of our work include:
\begin{itemize}[itemsep=0.2pt,topsep=0.2pt] %noitemsep can complete remove space between items
\item We propose a novel approach for latent augmentation that aims to build connections across samples from different domains by both \textit{degrading} and \textit{restoring} the samples from the latent distribution.
% using sample-to-sample relationships.
% We utilize sample-to-sample relationships in both processes with classifier guidance to encourage the mixing of samples across domains.

\item We conduct empirical studies to demonstrate that our approach improves class-level alignment of features, as well as the uniformity or spread of the data distribution. 
These two properties are shown to be strongly correlated with downstream task performance \cite{wang2020understanding}.
% to be useful for pre-training models for different downstream tasks.
% The results are further supported by our visualization of the nearest neighbors of generated latents.
% evaluation, where  


%\item We conduct various empirical studies to demonstrate the effectiveness of our approach.improves class-level alignment of features, as well as the uniformity or spread of the data distribution. These two metrics have been shown to be useful for pre-training models for different downstream tasks.

\item We extensively evaluate the robustness of our method on domain generalization benchmarks and medical imaging datasets with strong domain shifts, where we provide various ablations to better understand different components of the method. Finally, we further demonstrate the versatility of our augmentation method by applying it to a long-tail recognition task.

% \item We evaluate the robustness of our method on domain generalization benchmarks and medical imaging datasets with domain shift. We also provide various ablations to better understand the method. Finally, we demonstrate the versatility of our method by testing it on a long-tail recognition task.

\end{itemize}

%\zkn{Much better intro! Just needs a bit more precise language tying some of the claims (e.g. sample-to-sample relationships) to elements of the method. Maybe a good framing is: 1) Inspired by diffusion, we propose a degradation/restoration process, 2) Addressing limitations of simple sample-to-sample mixing in prior works, we leverage batch-level sample-to-sample mixing through self-attention to perform this degradation/restoration, 3) Crucially, the restoration process is conditioned on the non-corrupted latents, using sample-to-sample relationships including to non-corrupted latents. This story is kind of there, but without the flow and not as explicitly/directly stated in many places. }


==> texts/intro_feb28.tex <==

\section{Introduction}
% Machine learning models are designed to learn patterns and relationships from training data in order to make predictions on new, unseen data. However, models trained on data from one particular domain may not perform well on data from other domains, which is known as the problem of domain generalization. This is especially challenging when the available training data is limited, which is often the case in real-world applications.

%Within the last few decades, deep learning methods have demonstrated outstanding performance in extracting patterns and relationships from training data in various fields of computer vision. However, machine learning systems are often vulnerable to domain shifts, 
%where the performance of models would drop significantly when testing data are statistically different from training data. 
%The problem of generalizing on data from new, unseen domains is known as domain generalization (DG),
%which is an especially critical, but challenging, problem when the available training data is limited, which is often the case in real-world applications.

% I asked ChatGPT to rewrite this for me and I am quite happy about the results?
Over the past few decades, deep learning techniques have shown remarkable results in identifying patterns and correlations from training data in various fields of computer vision. However, machine learning systems are frequently prone to domain shifts, wherein their performance drastically drops when the testing data is statistically different from the training data. The issue of generalizing to data from new and unseen domains is referred to as domain generalization (DG), which is a particularly critical, but challenging issue, especially when the available training data is limited, as is often the case in real-world applications.


To address the problem of domain generalization, various methods have been proposed, such as feature alignment approaches \cite{sun2016deep}, meta-learning \cite{sankaranarayanan2023meta,balaji2018metareg}, and augmentation methods \cite{zhou2021domain}. % Feature alignment methods attempt to align the distributions of different domains to make them more similar, while metalearning methods aim to learn from multiple domains in order to improve generalization performance. 
%\zkn{Would be good to have references throughout this paragraph}
%Among the existing augmentation methods,
%data augmentation methods generate new samples by applying transformations to the existing ones, which can help models learn more robust and invariant features. 
However, many methods in DG typically require domain information, either to guide their generation of novel or adversarial samples (CITE), or to build domain invariant representations ((CITE). However, this can be limiting in cases where we don't have explicitly defined domains or have datasets that span a large number of related domains (ex: ). Thus, new approaches are needed for improving generalization that don't require explicit information about the underlying domains to guide training.
%\zkn{Can you explicitly describe what the disadvantages of these are (extra information used, computation, etc.)}. 

%One general approach for improving model generalization that has shown promise in a wide range of applications is augmentation. Latent augmentation approaches like Manifold-Mixup (CITE) and i-Mixup (CITE) instead, mix style statistics or adding noise into the latent space. 
%However, existing latent augmentation methods that use pairwise mixtures of samples (mixup)
%typically work better in small-scale settings, while when having a larger dataset or a larger backbone, they do not demonstrate sufficient and consistent improvement.
%\zkn{Would be nice to have something about addition of inference parameters to start building the case against MIRO}
% However, despite these efforts, achieving robust out-of-domain generalization remains a difficult problem, and further research is needed to develop more effective methods.

\begin{figure}[t!]
\centering
  \includegraphics[width=0.49\textwidth]{images/Fig1_ran_edit.png}
  \caption{\footnotesize {\em Visualization of latent degradation and restoration steps during training.} In (A), we visualize the degradation and restoration steps for a single class early in training when samples from different domains are separated. For a single query point, we simulate different possible augmentations generated by our model. In (B), we visualize the latents at a later point in training and color data by classes.\label{fig:fig1}}
\end{figure}

%With this in mind, we propose a novel approach for latent augmentation that aims to improve out-of-domain generalization. 
% In this paper, we propose a novel approach for latent augmentation that provides consistently better performance over the augmentation-based state-of-the-art for out-of-domain generalization
In this paper, we propose a novel latent augmentation approach for improving out-of-domain generalization. 
Our approach is loosely inspired by diffusion models \cite{ho2020denoising,rombach2022high}, in that the goal is bi-directional.
%to a noisy version of itself and reversing the process, one can \textit{restore} the semantic structure of the data, and generate diverse samples for training (see Figure~\ref{fig:fig1}A).
To ensure the generated samples would produce information that is robust to new domains,
% To achieve that,
we introduce a distribution-aware degradation to the original samples based on sample-to-sample relationships, with the aim of confusing the classifier. In the restoration stage, we use a permutation-invariant cross-attention mechanism to recover the original class, which conditions on the original latents and uses degraded latents as queries. By building relationships across samples, the restoration stage encourages the latents to connect across domains,
%\zkn{What does ``connect across domsin'' mean?}, 
leading to better generalization performance when facing an unseen domain. 

% \zkn{This evaluation part should go in next paragraph}We evaluate the effectiveness of our proposed method on several benchmark datasets and compare it with existing state-of-the-art methods. Our results demonstrate that the proposed approach improves out-of-domain generalization and achieves better performance than existing methods.

To demonstrate the utility of our approach and its wide range of potential applications, we conduct experiments on (i) five standardized domain generalization benchmarks \cite{gulrajani2020search,cha2021swad},
(ii) five medical imaging classification datasets that suffer from
domain shifting issues \cite{koh2021wilds,yang2023medmnist}\zkn{Emphasize low-labeled?}, and (iii) a long-tail recognition task where class imbalance is present \cite{hou2022batchformer}\zkn{Would be good to connect these; what does long-tail have to do with DG? Maybe pose generalization problem in long-tailed. }. 
In all of these cases, we show significant improvements with our approach over the baseline\zkn{May want to lead with next part (gain over other augmentation methods) rather than doing better than baselines}, and provide impressive boosts over other augmentation-based approaches on all the datasets tested. To further quantify the impact that our approach has on learning, we used uniformity and alignment \cite{wang2020understanding}\zkn{Provide short intuition as to what these are} to understand the latent quality, and used nearest neighbor visualization to understand how the data augmentation is taking effect. 
\zkn{This last sentence seems redundant}Our results demonstrate the effectiveness of the proposed approach and its potential for improving the robustness and generalization of deep learning models in real-world applications.



%A flexible and general mechanism underlying many of these methods is {\em data augmentation}, or the introduction of noise (CITE) or other in-context generators (CITE) to expand the distribution of the data seen during training. For instance, simple data augmentation methods such as Mixup and Cutmix (\cite{zhou2021domain}) have been successful in generating synthetic samples that improve learning, both through smoothing the decision boundary of the model, and creating soft adversaries during training \cite{zhang2020does}. More advanced data-adaptive approaches have also been proposed, many of them trying to adapt noise parameters or metalearning a good generative model to map between different domains. Despite this progress, generating good augmentations that can improve out-of-domain generalization remains an open challenge. 


% In this paper, we propose a novel latent augmentation method that tries to first {\em degrade} and then {\em restore} the latents during training. 
% For the degradation stage, we leverage sample-to-sample relationships to generate meaningful degradation of original samples that aims to confuse the classifier. 
% For the restoration stage, the aim is again to use information between samples, but now to recover the original class. We do this with a cross-attention mechanism, where we use the degraded latents as the queries and condition on the original latents. This restoration stage not only provides the classifier with more diverse and challenging samples to learn, but through building relationships across samples, the restoration stage encourages the latents to build connections across domains, and thus provide better generalization performance when facing unseen domain.


The contributions of our work include:
\begin{itemize}
% \item We propose a novel approach for distribution-aware augmentation that combines a latent degradation and restoration process as an effective latent augmentation operation, which can be applied to domain generalization and other tasks where domain shift and class imbalance occur.

\item We propose a novel approach for latent augmentation that 
% relies on sample-to-sample relationships, which 
aims to combine the \textit{degradation} and \textit{restoration} process to
build connections across samples from different domains to improve model generalization.
% and can be applied to domain generalization and other tasks where domain shift and class imbalance occur.
\item We utilize sample-to-sample relationships to design the latent \textit{degradation} and \textit{restoration} process, and use classifier guidance to further encourage the mixing of samples across domains. 
% We designed different stochastic ways to guide the degradation process, and used a cross-attention transformer for the restoration process.
\item We demonstrate the robustness of our method on domain generalization benchmarks and medical imaging datasets with strong domain shifting, and provide various ablations, visualizations, and latent quality evaluation metrics to understand the proposed method. The method is further tested on a long-tail recognition task, which shows the versatility of the method.
\end{itemize}


\zkn{Overall the intro reads well and highlights everything nicely! Nice job putting it together.  A few key things include: 1) Adding more intuition and precise details as to your approach, 2) Having a consistent set of claims about how you're better (e.g. compared to other augmenation methods, without use of additional parameters during inference, etc.).}






==> texts/intro_march4.tex <==
\section{Introduction}

Over the past few decades, deep learning techniques have shown remarkable progress in various fields of computer vision \cite{he2016deep,guo2018review}. However, machine learning systems are frequently prone to domain shifts, wherein their performance  drops when the testing data is  different from the training data \cite{csurka2017domain}. This is a critical issue in real-world applications where training data may be limited. Despite recent advances, domain generalization remains a challenging task that requires new approaches to achieve robust and reliable performance \cite{gulrajani2020search}.

To address the problem of domain generalization, various methods have been proposed, such as feature alignment approaches \cite{sun2016deep,sun2016deep,wang2020domainmix}, meta-learning \cite{sankaranarayanan2023meta,balaji2018metareg}, and augmentation methods \cite{zhou2021domain,hong2021stylemix,li2021simple}. 
However, many methods in DG don't use sample-to-sample level information. 
Thus, new approaches are needed for improving generalization in challenging new domains.

\begin{figure}[t!]
\centering
  \includegraphics[width=0.49\textwidth]{images/Fig1_ran_edit.png}
  \caption{\footnotesize {\em Visualization of latent degradation and restoration steps during training.} In (A), we visualize the degradation and restoration steps for a single class early in training when samples from different domains are separated. For a single query point, we simulate different possible augmentations generated by our model. In (B), we visualize the latents at a later point in training and color data by classes.\label{fig:fig1}}
\end{figure}


In this paper, we propose a novel latent augmentation approach for improving domain generalization. Our approach works without any assumptions on training or testing domains, and doesn't require additional parameters at inference. To build our latent augmentation approach, we take inspiration from diffusion models \cite{ho2020denoising,rombach2022high} and define two operations: one that aims to degrade the latents by mapping them to a different noisy class label, and the second to restore the latents back to their original classes. 
In both stages, we use the embeddings from other samples in the mini-batch to transform each query sample, and thus we use the sample-to-sample relationships across the latent distribution during training. In the restoration stage, we use a permutation-invariant cross-attention mechanism (CITE), which conditions on the original latents and uses degraded latents as queries. 
%Each query sample thus is associated with a triplet: the original latent, the augmented latent after degradation, and the latent after restoration. We can thus think about this process through a contrastive lens where we define two samples as positive examples (original, restored) and the third degraded sample as a negative example.

%By encouraging the latents to be mapped back to the original class but not necessarily be mapped back to their original position in the latent space, the restoration stage can generate augmentations that map  other domains, leading to better generalization performance when facing an unseen domain. 

To demonstrate the utility of our approach in diverse settings, we conduct experiments on: (i) five standardized domain generalization benchmarks \cite{gulrajani2020search,cha2021swad},
(ii) five medical imaging classification datasets that suffer from 
domain shifting issues \cite{koh2021wilds,yang2023medmnist}, and (iii) a long-tail (LT) recognition task where class imbalance is present \cite{hou2022batchformer}.  
In all of these cases, we provide impressive boosts over other augmentation-based approaches on all the datasets tested, and competitive performance with state-of-the-art methods that use more complex losses and domain information. To further quantify the impact that our approach has on learning, we used two measures of representation quality \cite{wang2020understanding} and used nearest neighbor visualization to understand how the data augmentation is taking effect. 
%\zkn{This last sentence seems redundant}Our results demonstrate the effectiveness of the proposed approach and its potential for improving the robustness and generalization of deep learning models in real-world applications.


The contributions of our work include:
\begin{itemize}
\item We propose a novel approach for latent augmentation that 
aims to combine the \textit{degradation} and \textit{restoration} process to
build connections across samples from different domains. 
We utilize sample-to-sample relationships in both the latent degradation and restoration process, and use classifier guidance to further encourage the mixing of samples across domains. 

\item We analyze the latent representations obtained via our approach and compare with other methods. We show that our approach improves the class-level alignment of features while also improving the uniformity and overall spread of the data distribution, two features that have been shown to be useful in pre-training for different downstream tasks.

\item We demonstrate the robustness of our method on domain generalization benchmarks and medical imaging datasets with  domain shift, and provide various ablations to understand the method. The method is further tested on a long-tail recognition task, which shows the versatility of the method.
\end{itemize}





==> texts/method_Feb17.tex <==
\section{Method}

% \subsection{Background}

\subsection{Transformer basics}

\paragraph{Attention mechanism}

% please remember to edit text, copied from EIT

When having sequences of inputs $X = [\mathbf{x}^{1}\ \mathbf{x}^{2}\ \dots \  \mathbf{x}^{N}]^T \in \mathbb{R}^{N \times d}$ that consists of $N$ tokens of $d$-dimensions,
the self-attention mechanism learns the relationship between elements inside sequence through deriving queries $Q$, keys $K$, and values $V$ by performing linear projections for each token embedding as below:
\[
Q = XW_Q, K = X W_K , V = X W_V
\]
where $Q \in \mathbb{R}^{N \times d_q}$, $K \in \mathbb{R}^{N \times d_k}$, $V \in \mathbb{R}^{N \times d_v}$. The self-attention is built by performing multiplication of the key, query, and values. It can be viewed as using the query to 
\begin{equation}
\label{eq:attention}
    \operatorname{Attention}(Q,K,V) = \operatorname{softmax}\left( \frac{1}{\sqrt{d_k}}{Q K^{T}}\right) V,
\end{equation}
where $\operatorname{softmax}(\cdot)$ gives row-wise softmax normalization.

\paragraph{Conditioning with cross attention}

The attention mechanism can also handle inputs from different sources or modalities. Given $X_1 = [\mathbf{x_1}^{1}\ \mathbf{x_1}^{2}\ \dots \  \mathbf{x_1}^{N}]^T \in \mathbb{R}^{N \times d_1}$ and $X_2 = [\mathbf{x_2}^{1}\ \mathbf{x_2}^{2}\ \dots \  \mathbf{x_2}^{N}]^T \in \mathbb{R}^{N \times d_2}$, the queries $Q$, keys $K$, and values $V$ are computed from different sources:
\[
Q = X_1W_Q, K = X_2 W_K , V = X_2 W_V
\]
This cross-attention mechanism is shown to be effective when performing conditioning \cite{rombach2022high}. As the attention mechanism is permutation-invariant, the ordering of the output would be decided based on the ordering of the queries ($X_1$), while the condition ($X_2$) serves as the knowledge bank. From the perspective of content style separation, the queries provide the content, while the condition provides the style.

% would produce  attention operation 


\paragraph{Transformer encoder}

The transformer architecture is built based on the attention mechanism (AttN), MLP blocks (FF), and layerwise normalization (LN). The operations are:
\begin{equation}
\label{eq:MSA}
\begin{aligned}
    & Z_{\ell+1}^{\prime} = \operatorname{LN}(Z_{\ell} + \operatorname{AttN}(Z_{\ell})) \\
    & Z_{\ell+1} = \operatorname{LN}(Z_{\ell+1}^{\prime} + \operatorname{FF}(Z_{\ell+1}^{\prime})), ~0 \leq \ell \leq L-1
\end{aligned}
\end{equation}
When having conditions, the operations remain unchanged, but the attention mechanism is replaced as below:
\[
\operatorname{AttN}(Z_{\ell}) \Rightarrow \operatorname{Cross-AttN}(Z_{\ell}, X_2)
\]
where $X_2$ would serve as an order-less condition to assist the learning process.

% When feeding the network pairs of data points $X_1$ and $X_2$, and using cross-attention instead of self-attention, the operation becomes as below:
% \paragraph{MetaTransformer}

Recently, \cite{yu2022metaformer} shows that the self-attention operation can be replaced by spatial MLP, or Pooling operations for images, which would maintain robust performance while reducing the computation complexity.
\[
\operatorname{AttN}(Z_{\ell}) \Rightarrow \operatorname{Spatial-MLP}(Z_{\ell}) \text{ or } \operatorname{Pooling}(Z_{\ell})
\]
% where $\operatorname{Mixing}$ can be any mixing operation, which can be a simpler spatial MLP, or even a parameter-less operation as the Pooling operation.


\subsection{Our method}

\paragraph{Overview}

Our method aims to exploit the relationship between samples through the process of degradation and restoration.
The process is inspired by \cite{bansal2022cold}.
Consider $x \in \mathbb{R}^N$ as an original datapoint, our method is built by a degradation operator $D$ to create an augmented sample $x_{\operatorname{d}}$, and a restoration operator $R$ that (approximately) inverts $D$.
\[
R\left(x_{\operatorname{d}}\right) \approx x
\]

In most of the traditional works, the degradation operator and the restoration operator are trained by the below minimization problem that operates directly on the data space:
\[
\min _{\theta, \mu} \mathbb{E}_{x \sim \mathcal{X}}\left\|R_\theta(D_{\mu}(x))-x\right\|,
\]
where $x$ denotes a random image sampled from the data distribution $\mathcal{X}$ and $\|\cdot\|$ denotes a norm, which is mostly $\ell_1$ or $\ell_2$. % We can use the subscript $R_\theta$ to emphasize the dependence of $R$ on $\theta$ during training.

% In the real diffusion models, the diffusion process needs to be performed sequentially, because when having a large $t$, the restoration network $R_\theta$ loses its power. There are many ways to address it via designing new scheduler, but still, the most state-of-the-art diffusion model still would need many steps (iterations) to generate high-resolution images.


\paragraph{Sample-aware operators}

When designing the degradation operator, we would like the operator to consider sample-to-sample relationship. Specifically, we consider the model training process under the mini-batch setting, where for each sample $\mathbf{x}$, we would consider fetch a batch of random samples $X_b$ ($\mathbf{x} \in X_b$):
\[
x_{\operatorname{d}} = D(\mathbf{x} \mid X_b)
\]
where we use a random batch of samples to control both the severity and the direction of the production of $\mathbf{x}_{\operatorname{d}}$.

Similarly, when having the restoration operator $R$, we consider the process:
\[
R\left(x_{\operatorname{d}} \mid X_{b} \right) \approx x
\]
Specifically, we use a transformer encoder with cross attention to perform the restoration process. 
By using a transformer with cross attention, $X_{b}$ is presented to the encoder as an order-less batch of samples, while $x_{\operatorname{noise}}$ takes the responsibility to find the best match as queries.

\paragraph{Classifier-guidance}

% Instead of optimizing the below function:
% \[
% \min _{\theta, \mu} \mathbb{E}_{x \sim \mathcal{X}}\left\|R_\theta(D_{\mu}(x))-x\right\|,
% \]

We use the classifier $g(\cdot)$ and loss function $\ell(\cdot, \cdot)$ to perform guidance, to optimize the below function:
\[
\min _{\theta, \mu} \mathbb{E}_{x \sim \mathcal{X}} \ell(g(x), y) + \mathbb{E}_{x \sim \mathcal{X}} \ell(g(R_\theta(D_{\mu}(x)), y)
\]
Thus, the restoration is relaxed, such that the restoration is regularized such that it will return to the original distribution of labels instead of the original distribution of itself.

The second term is to minimize the below risk:
\[
R = \int \ell(g(x), y) \mathrm{d} P(x^{\operatorname{recover}}, y)
\]
where $\left(x_{i}^{\operatorname{recover}}, y_i\right) \sim P$ is a more diverse set of samples than the distribution of the original data $\left(x_{i}, y_i\right) \sim P$.

\textit{Remark. Consider the domain generalization setting, where the same label $y$ could map to $x_1$ and $x_2$ from two different distributions, this classifier-guided (soft) process of latent restoration might allow the restoration of $x_1$ to $x_2$.}


\paragraph{Building soft-label for degraded samples}

In order to make sure that $\left(x_{i}^{\operatorname{recover}}, y_i\right) \sim P$ provides a more diverse set of samples, we need to first ensure the degradation provides a diverse set of samples. In order to provide a diverse set of noisy samples, we regularize the degraded samples to be aligned with soft labels as below:
\[
y_{\operatorname{soft}} = \frac{1}{B} \sum_{y_i \in Y_b} y_i
\]
Thus, we optimize the below function:
\[
\min _{\theta, \mu} \mathbb{E}_{x \sim \mathcal{X}} \ell(g(D_{\mu}(x), y_{\operatorname{soft}})
\]
By doing so, we are creating samples that are not only diverse, but also confusing to the classifier.

Specifically, mixup was using the below distribution created by convex optimization:
\[
\begin{aligned}
&\mu\left(\tilde{x}, \tilde{y} \mid x_i, y_i\right) = \\
&\frac{1}{n} \sum_j^n \underset{\lambda}{\mathbb{E}}\left[\delta\left(\tilde{x}=\lambda x_i+(1-\lambda) x_j, \tilde{y}=\lambda y_i+(1-\lambda) y_j\right)\right]
\end{aligned}
\]
our formulation, instead, consider the mini-batch distribution directly with the alternative distribution:
\[
\begin{aligned}
&\mu\left(\tilde{x}, \tilde{y} \mid x_i, y_i\right) = \\
&\frac{1}{n} \sum_j^n \underset{\lambda}{\mathbb{E}}\left[\delta\left(\tilde{x}=D_\theta (x_i \mid X_b), \tilde{y} = \operatorname{average}(Y_b) \right)\right]
\end{aligned}
\]
which creates a non-convex combination of samples following the distribution $\mu(\tilde{x}, \tilde{y})$. This distribution is later used in the restoration operator to generate a diverse set of $x^{\operatorname{recover}}$.

\paragraph{Summary}

To summarize, our algorithm is built based on both the batch-wise nonconvex mixture of samples to perform latent degradation, as well as the classifier-guided latent restoration. The algorithm can be easily implemented as 7 lines of code as in pseudocode \ref{code:alg} as a pluggable term during training.

\begin{algorithm}[h]
\label{code:alg}
\SetAlgoLined
    % \PyComment{going to have indentation} \\
    \PyCode{def train(l, y, g, ft, bt):} \\
    \Indp   % start indent
        % \PyComment{l: latent} \\
        % \PyComment{y: label} \\
        \PyCode{l$_f$ = ft(l)} \\ % \PyComment{inline comment} \\ 
        \PyCode{l$_b$ = bt(l$_f$, l)} \\
        \PyCode{y$_{soft}$ = average(y)} \\
        \PyCode{loss1 = criteria(g(l), y)} \\
        \PyCode{loss2 = criteria(g(l$_f$), y$_{soft}$)} \\
        \PyCode{loss3 = criteria(g(l$_b$), y)} \\
        \PyCode{loss = loss1 + loss2 + loss3} \\   
        \PyCode{loss.backward()} \\
    \Indm % end indent, must end with this, else all the below text will be indented
%    \PyComment{this is a comment} \\
%    \PyCode{your code}
\caption{PyTorch-style pseudocode}
\label{algo:your-algo}
\end{algorithm}


%\subsection{Understanding the method through the lens of content/style separation of classifier}
% \paragraph{Additional back translation for cycle consistency} 

% We provide an intuitive explanation of the method from the perspective of content/style separation of the latent space. Intuitively, for the domain generalization perspective, each sample from the dataset should contain three parts of information: (1) The class-related property, which is one specific type of mutual information, that is learned by minimizing the loss of classifier. (2) The domain-related property, which is the `style', a classifier that should be ignored by the classifier, but in the domain generalization setting there are few `styles' that are obvious to the learning process. (3) Instance-specific variance.


\subsection{Evaluate latents with alignment and uniformity}

To further understand how the proposed method would encourage the latent representation to help in terms of generalization (robust to domain shifting) and classification (clustering of the same class), we used the latent representation evaluation methods proposed in \cite{wang2020understanding}.

Specifically, latent representation can be evaluated through the lens of alignment and uniformity. Alignment measures the `closeness' of features from the same class; while uniformity measures the distribution of the (normalized) features on
the hypersphere, which can be understood as the diversity of samples. The metrics are as below:
\[
\begin{aligned}
& \mathcal{L}_{\text {align }}(f ; \alpha) \triangleq \mathbb{E}_{(x, y) \sim p_{\text {pos }}}\left[\|f(x)-f(y)\|_2^\alpha\right] \\
& \mathcal{L}_{\text {uniform }}(f ; t) \triangleq \log \mathbb{E}_{x, y \stackrel{\text { i.i.d. }}{\sim} p_{\text {data }}}\left[e^{-t\|f(x)-f(y)\|_2^2}\right] . \\
&
\end{aligned}
\]
As shown in \cite{wang2020understanding}, those two properties are desired properties in self-supervised representation learning works. To extend the use of the metrics, and to further understand how the representation in domain generalization settings can be evaluated beyond classification accuracy, we compare our methods with other methods based on those metrics.

==> texts/method_Feb25.tex <==
\section{Method}

% \subsection{Background}


\subsection{Overview of our method}

Inspired by diffusion models \cite{rombach2022high}, our data augmentation operation is learned through a {\em degradation} step and {\em restoration} step. 
% The learning of the degradation and restoration operators work hand in hand at the batch level. 
%Critically, after augmenting samples in the batch, we use cross-attention to query the sample using its relative position in the original latent distribution, using keys from the original latents to learn a back translation with queries from the augmented latents. 
We visualize both steps in our process in Figure~\ref{fig:fig1} and provide a overview of architecture in Figure~\ref{fig:arch}.
%Our algorithm is built based on both the batch-wise nonconvex mixture of samples to perform latent degradation, as well as the classifier-guided latent restoration. 
The method can be implemented easily and fit into the mini-batch training process and can be removed during inference. %It can also be used in conjunction with targeted augmentations or other domain generalization methods.


% \subsubsection{High-level Objective}~ 
Consider $(x, y)$ as an original datapoint and label pair from our data distribution $(\mathcal{X}, \mathcal{Y})$. Let $z = f(x)$ denotes the embedding of $x$ after the encoder $f$, and $g(z)$ as the classifier that produces final prediction.
% and $Z \in \mathbb{R}^{L \times B}$ contains the representations of a batch of samples from the dataset, where $L$ is the dimension of the latent space and $B$ is the size of the batch. 
The overall objective of the method is to learn a latent degradation operator $D_{\mu}$ that produces embeddings that would `confuse' the prediction of the labels; and a latent restoration operator $R_{\theta}$ that would `denoise' the prediction of the labels.
% denote the forward step to augment latents and let $R_{\theta}$ denote the reverse mapping that (approximately) inverts $D$ to produce a batch that is mapped back to their corresponding and correct labels. 
% In this work, we consider a supervised setting where we have labels $y$ and an appropriate loss function $\ell(\cdot, \cdot)$ that matches the prediction problem at hand (for instance, cross entropy). 
This high-level objective can be specified as:
%\[
%\min _{f, g, \theta, \mu} \mathbb{E}_{x \sim \mathcal{X}} ~ \ell(g(z), y) +  \ell(g(R_\theta(D_{\mu}(z)), y)
%\]
\[
\begin{aligned}
z_{d} = D_{\mu}(z) \centernot{\xRightarrow{g}} y ;\quad
z_{r} = R_\theta(D_{\mu}(z)) \xRightarrow{g} y
% \ell(g(z), y) \neq \ell(g(D_{\mu}(z)), y), \\
% \ell(g(z), y) \approx \ell(g(R_\theta(D_{\mu}(z)), y),
\end{aligned}
\]
% where $g$ is a classifier that is trained to predict the output labels $y$, and $D_{\mu}(z)$ introduces some non-trivial perturbation to the latent variables. 
Intuitively, this can be viewed as an adversarial process: while the restoration operator learns to predict the original distribution of labels; the degradation operator aims to introduce non-trivial perturbation to the latent variables such that it would alter the classifier's prediction.
% Through this process, the degradation operator aims to introduce non-trivial perturbation to the latent variables such that the method does not provide trivial solutions; while the restoration operator learns to return the latents back to their original distribution of labels. 
Note that different from other methods, our recovered latent $z_{r} = R_{\theta}(D_{\mu}(z))$ does not necessarily need to be close to its original position $z$ as long as the classifier's prediction is correct, which encourages the data to go across domains.

% In general, without appropriate constraints on the degradation, a trivial solution can be the identity, however, we will next describe a procedure to push the latents away from their original positions to ensure that this doesn't happen.

\subsection{Our method}

\subsubsection{Latent degradation with soft labels}

In order to encourage the datapoints from different domains to mix with each other and provide additional sample information during training, we construct new latent and label pairs $(\mathcal{Z}_{new}, \mathcal{Y}_{new})$ from the original distribution $(\mathcal{Z}, \mathcal{Y})$. 
% a latent sampling process and create soft labels to guide the learning process in the degradation step.

Specifically, % consider the whole latent distribution for all training data as $\mathcal{Z}$, and consider a latent embedding $z$ drawn from the distribution.
when drawing a latent embedding $(z, y) \sim (\mathcal{Z}, \mathcal{Y})$, we would like to have a subset $(\mathcal{Z}_{set}, \mathcal{Y}_{set})$, so that we can construct the below pairs:
% $z$ and its corresponding label $y$ can be augmented through the below sampling process:
\[
z_d \sim \operatorname{Mix}_{\text{data}}(z, \mathcal{Z}_{set}); \quad
y_d \sim \operatorname{Mix}_{\text{label}}(y, \mathcal{Y}_{set}),
\]
where $\operatorname{Mix}$ is a mysterious mixing operator.

% Basically, each $z$ would be augmented such that it would consider the mixture of a random subset of latent samples from the data distribution $\mathcal{Z}$ to obtain an augmented sample $z_d$.

% However, this sampling process could risk the storage expensive memory bank and is thus infeasible. To resolve this, we consider $\mathcal{Z}_b$ as a batch of latent embeddings, and use either a self-attention transformer with dropout or a pooling variant of it (inspired by PoolFormer \cite{yu2022metaformer}), which gives us the below latent degradation operator:


We implement $\operatorname{Mix}_{\text{data}}$ with two choices of transformers that focus on finding spatial correlations: 
\[
\begin{aligned}
& z_d \sim D(z_d \mid z) = \operatorname{Trans}(Z_{set}), \\ 
& \myrightarrow{SA} z^{\prime}_d = z + \operatorname{AttN}(Z_{set}), \\
& \myrightarrow{Pool} z^{\prime}_d = z + \operatorname{Pooling}(\operatorname{Subset}(Z_{set})),
\end{aligned}
\]
where $z^{\prime}_d$ is the first operator output of transformer layer \ref{eq:MSA}, which would layer be passed into an MLP with the residual connection.
The randomness is introduced through either the self-attention operation with dropout, or is introduced through a pooling and subset operation. 
% The actual Transformer layer also comes with layer normalization and MLP, as introduced in Method.

In terms of $\operatorname{Mix}_{\text{label}}$, we create the soft label as below:
\[
y_{\text{soft}} = \frac{1}{|\mathcal{Y}_{set}|}\sum_{y_{i} \in \mathcal{Y}_{set}} y_{i}
\]

By creating the $(\mathcal{Z}_{new}, \mathcal{Y}_{new})$ pairs as above, 
% In order to encourage this forward procedure to map the data to a common distribution that may encourage mixing of samples across different domains, 
we generate the degraded latents that are aware of other samples, and their corresponding soft or noisy labels. 
%We can write out the loss associated with our forward operation as:
%\[
%\mathcal{L}_{\text{degrade}} = \ell(g(D_{\mu}(z), y_{\operatorname{soft}})
%\]
%where $\ell()$ is a loss function of selection, which we used CrossEntropy.
% In practice, we set  $y_{soft} = \operatorname{average}(Y_b)$ to the average over all the one-hot labels in the batch. % However, we also test other label distributions in XX.
Note that this $\mathcal{Z}_{set}$ fits perfectly into mini-batch training, such that it can just be a batch of data that produces noised samples $\mathcal{Z}_{d}$.



\subsubsection{Latent restoration with cross-attention}~
% Having a degradation operator that tries to confuse the classifier, we still 
% Both the degradation  and restoration operators work together in tandem to ensure that the latents can be recovered. In other words, while performing latent degradation, we would like $z_{d}$ to still be distinguishable, or recoverable, such that it still contains the trace of the original $z$ and we can recover its class.
% Generating pure noise is not going to be helpful for the model to learn. 
Instead of letting the model learn pure noisy latent and label association, we would like to ask the model to have the capability to trace back the remaining information inside a noised latent.
In other words, we want the model to be robust such that even if there is noise injected, it can still leave a trace in the latent space such that it can potentially be recovered.
% In other words, we would like to enforce the degradation operator to generate both confusing samples, and traceable samples. 
Thus, we perform a latent restoration step that aims to distinguish or recover $z_{d}$ such that we can recover its class information.% to still be distinguishable, or recoverable, such that it still contains the trace of the original $z$ and we can recover its class.

To restore the latents back to their original classes, our model leverages a cross-attention mechanism that computes queries $Q$ from the corrupted latents $\mathcal{Z}_d$ and the keys $K$ and values $V$ from the original latents $\mathcal{Z}_{set}$:
%\[
%Q = Z_B W_Q, K = Z_{corr} W_K , V = Z_{corr} W_V
%\]
\[
Q = \mathcal{Z}_d W_Q, K = \mathcal{Z}_{set} W_K , V = \mathcal{Z}_{set} W_V
\]
As the attention mechanism is permutation-invariant, the ordering of the output would be decided based on the ordering of the queries, which enforces the corrupted latents to contain the information that is enough to recover the class of the original latents. % At the same time, $Z$ serves as a knowledge bank. 
% The intuition behind this is XX and YY.
Thus, intuitively, 
% the restoration operator is learning to (approximately) invert the augmentations based on cross-attention:
the restoration operator generates a new latent with the same class information based on the trace that left by the degradation process:
\[
\begin{aligned}
& z_r \sim R(z_{r} \mid z_{d}) = \operatorname{Trans}(\mathcal{Z}_b \mid \mathcal{Z}_{set}), \\
& \myrightarrow{CA} z^{\prime}_{r} = z_d + \operatorname{softmax}(QK^T) V
\end{aligned}
\]
where the corrupted latents select similar samples from the original latents and construct new latents. Thus, we created new latent and label pairs $(\mathcal{Z}_r, \mathcal{Y})$.
% Similar as above, instead of using a reconstruction loss, we rely on classifier guidance to regularize the reverse process. 
% This relaxed regularization process aims to encourage samples from different domains to be mapped to their corresponding class during restoration, thus creating a type of domain-invariance and more robustness in the classification task.


\subsubsection{Regularization with classifier guidance}

Thus, for each sample $z$, we created three latent and label pairs. $(z, y)$ as the original ones, $(z_b, y_{\text{soft}})$ as the degraded ones, and $(z_r, y)$ as the restored ones. We perform a relaxed regularization with classifier guidance, where our model aims to optimize the below combined loss:
% our method aims to optimize a combination of the following three losses:
\[
\mathcal{L} =  \underbrace{\ell(g(z), y)}_{\text{original}} + \underbrace{ \ell(g(R_\theta(D_{\mu}(z)), y)}_{\text{restore}} + \underbrace{\ell(g(D_{\mu}(z), y_{\operatorname{soft}})}_{\text{degrade}}
\]
where $\ell$ is a classification loss function (e.g. CrossEntropy).

There are two key properties of our proposed method: Firstly, we rely on the classifier to both guide the corrupted latents towards misclassification and back to their correct labels after restoration. This provides a soft constraint that encourages the latent embeddings to be flexible. Secondly, the operations use the population distribution of samples within batch to both create degraded samples and also restored samples, and this usage of sample-to-sample relationships benefits the training. Our method can fit perfectly into mini-batch training, as shown in pseudocode in Algorithm~\ref{algo:main}.

% \subsection{Discussion of method and comparisons}
% Mixup was using the below distribution created by convex optimization:
% \[
% \begin{aligned}
% &\mu\left(\tilde{x}, \tilde{y} \mid x_i, y_i\right) = \\
% &\frac{1}{n} \sum_j^n \underset{\lambda}{\mathbb{E}}\left[\delta\left(\tilde{x}=\lambda x_i+(1-\lambda) x_j, \tilde{y}=\lambda y_i+(1-\lambda) y_j\right)\right]
% \end{aligned}
% \]
% our formulation, instead, consider the mini-batch distribution directly with the alternative distribution:
% \[
% \begin{aligned}
% &\mu\left(\tilde{x}, \tilde{y} \mid x_i, y_i\right) = \\
% &\frac{1}{n} \sum_j^n \underset{\lambda}{\mathbb{E}}\left[\delta\left(\tilde{x}=D_\theta (x_i \mid X_b), \tilde{y} = \operatorname{average}(Y_b) \right)\right]
% \end{aligned}
% \]
% which creates a non-convex combination of samples following the distribution $\mu(\tilde{x}, \tilde{y})$. This distribution is later used in the restoration operator to generate a diverse set of $x^{\operatorname{recover}}$.




%From the perspective of content style separation, the queries provide the content, while the condition provides the style.


%Putting this together, we have the following loss:
%\[
%\min_{g, f, \theta, \mu}  g( z, y) + g( R_{\theta}\left( D_{\mu} ( z , Z_B ) , \widetilde{Z_B} \right), y), 
%\]



%In most of the traditional works, the degradation operator and the restoration operator are trained by the below minimization problem that operates directly on the data space:
%\[
%\min _{\theta, \mu} \mathbb{E}_{x \sim \mathcal{X}}\left\|R_\theta(D_{\mu}(x))-x\right\|,
%\]
%where $x$ denotes a random image sampled from the data distribution $\mathcal{X}$ and $\|\cdot\|$ denotes a norm, which is mostly $\ell_1$ or $\ell_2$. % We can use the subscript $R_\theta$ to emphasize the dependence of $R$ on $\theta$ during training.

% In the real diffusion models, the diffusion process needs to be performed sequentially, because when having a large $t$, the restoration network $R_\theta$ loses its power. There are many ways to address it via designing new scheduler, but still, the most state-of-the-art diffusion model still would need many steps (iterations) to generate high-resolution images.


%In what we have described until now, we use the 

%We use the classifier $g(\cdot)$ and loss function $\ell(\cdot, \cdot)$ to perform guidance, to optimize the below function:
%\[
%\min _{\theta, \mu} \mathbb{E}_{x \sim \mathcal{X}} \ell(g(x), y) + \mathbb{E}_{x \sim \mathcal{X}} \ell(g(R_\theta(D_{\mu}(x)), y)
%\]
%Thus, the restoration is relaxed, such that the restoration is regularized such that it will return to the original distribution of labels instead of the original distribution of itself.

%he second term is to minimize the below risk:
%\[
%R = \int \ell(g(x), y) \mathrm{d} P(x^{\operatorname{recover}}, y)
%\]
% where $\left(x_{i}^{\operatorname{recover}}, y_i\right) \sim P$ is a more diverse set of samples than the distribution of the original data $\left(x_{i}, y_i\right) \sim P$.
% \textit{Remark. Consider the domain generalization setting, where the same label $y$ could map to $x_1$ and $x_2$ from two different distributions, this classifier-guided (soft) process of latent restoration might allow the restoration of $x_1$ to $x_2$.}
%\paragraph{Building soft-label for degraded samples}
%In order to make sure that $\left(z_{i}^{\operatorname{rec}}, y_i\right) \sim P$ provides a more diverse set of samples, we need to first ensure the degradation provides a diverse set of samples. 



%\subsection{Understanding the method through the lens of content/style separation of classifier}
% \paragraph{Additional back translation for cycle consistency} 

% We provide an intuitive explanation of the method from the perspective of content/style separation of the latent space. Intuitively, for the domain generalization perspective, each sample from the dataset should contain three parts of information: (1) The class-related property, which is one specific type of mutual information, that is learned by minimizing the loss of classifier. (2) The domain-related property, which is the `style', a classifier that should be ignored by the classifier, but in the domain generalization setting there are few `styles' that are obvious to the learning process. (3) Instance-specific variance.




\subsection{Assessing representation quality with alignment and uniformity metrics}

To assess the quality of representations learned through our model, we use two metrics shown to have good correlation with accuracy of classification from pre-trained models \cite{wang2020understanding}.  The first metric is the {\em alignment score}, a measure of the `closeness' of features from the same class. The second metric is the {\em uniformity score}, a measures the distribution of the (normalized) features on
the hypersphere and captures how well the representations span the space.
% , which approximates the diversity of the samples.

The alignment score is defined as:
\begin{equation}
\mathcal{L}_{\text {align }}(f) \triangleq \mathbb{E}_{(x_1, x_2) \sim p_{\text {cls }}}\left[\|f(x_1)-f(x_2)\|_2^2\right],
\end{equation}
where $(x_1, x_2) \sim p_{\text {cls}}$ draws samples from the same class.

The uniformity score is defined as:
\begin{equation}
\mathcal{L}_{\text {uniform }}(f) \triangleq \log \mathbb{E}_{x_1, x_2 \stackrel{\text { i.i.d. }}{\sim} p_{\text {data }}}\left[e^{-2\|f(x_1)-f(x_2)\|_2^2}\right],
\end{equation}
where in this case the samples $(x_1, x_2)$ are across the entire dataset, which demonstrates the generalization ability of the method as the model preserves the `maximal' available information from the training data.

% and $t=2$ sets the bandwidth of our radial basis function used to measure distance.

%As shown in \cite{wang2020understanding}, those two properties are desired properties in representation learning. 
%To extend the use of the metrics, and to further understand how the representation in domain generalization settings can be evaluated beyond classification accuracy, we compare our methods with other methods based on these metrics.

==> texts/method_Feb7.tex <==
\section{Method}

We introduce the method BatchTranslator in this section, and some corresponding visualization methods (?).

\subsection{Transformer basics}

\paragraph{Self-attention}
% \subsection{Transformer basics}

% please remember to edit text, copied from EIT
Transformers consider sequences of data in the format of $X = [\mathbf{x}^{1}\ \mathbf{x}^{2}\ \dots \  \mathbf{x}^{N}]^T \in \mathbb{R}^{N \times d}$ consisting of $N$ tokens of $d$-dimensions.
The self-attention mechanism derives queries $Q$, keys $K$, and values $V$ by performing linear projections for each token embedding, which gives $Q = XW_Q, K = X W_K , V = X W_V $, where $Q \in \mathbb{R}^{N \times d_q}$, $K \in \mathbb{R}^{N \times d_k}$, $V \in \mathbb{R}^{N \times d_v}$. The self-attention gives:
\begin{equation}
\label{eq:attention}
    \operatorname{Attention}(Q,K,V) = \operatorname{softmax}\left( \frac{1}{\sqrt{d_k}}{Q K^{T}}\right) V,
\end{equation}
where $\operatorname{softmax}(\cdot)$ gives row-wise softmax normalization.


\paragraph{Cross-attention}
Instead, cross-attention, which was briefly mentioned in \cite{vaswani2017attention}, later find its usage in \cite{jaegle2021perceiver} and \cite{rombach2022high}, considers two sequences $X_1 = [\mathbf{x_1}^{1}\ \mathbf{x_1}^{2}\ \dots \  \mathbf{x_1}^{N}]^T$ and $X_2 = [\mathbf{x_2}^{1}\ \mathbf{x_2}^{2}\ \dots \  \mathbf{x_2}^{N}]^T$ (which might be of different shapes, or different dimension $d$), and learns:
\[
Q= X_1 W_Q, K= X_2 W_K, V= X_2 W_V
\]
where $W_Q$ is the same as previous, but $W_K$ and $W_V$ are learnable projection matrices from the data that is being cross-attention-ed. In StableDiffusion \cite{rombach2022high} and other works, cross-attention is typically used as a general-purpose conditioning mechanism across different modalities, such as language prompts.

\paragraph{Transformer}

% please remember to edit text, copied from EIT
The transformer architecture as a model building block consists of many ($L$) layers of the below operations:
\begin{equation}
\label{eq:MSA}
\begin{aligned}
    & Z_0 =\left[\mathbf{x}^{1}, \mathbf{x}^{2}, \cdots \mathbf{x}^{N}\right]+\mathbf{E}_{\text {pos}} \\
    & Z_{\ell+1}^{\prime} = Z_{\ell} + \operatorname{Attention}(Z_{\ell}) \\
    & Z_{\ell+1} = Z_{\ell+1}^{\prime} + \operatorname{FF}(Z_{\ell+1}^{\prime}), ~0 \leq \ell \leq L-1
\end{aligned}
\end{equation}
where $Z_0$, as the initialization, sums up the individual token embedding and their positional embedding $\mathbf{E}_{\text {pos}}$ (which is optional, and not used in our architecture). Each transformer layer is the combination of the Attention operation ($\operatorname{Attention}(\cdot)$), the nonlinear projection ($\operatorname{FF}(\cdot)$, stands for feedforward network or MLP), and residual connections.

When feeding the network pairs of data points $X_1$ and $X_2$, and using cross-attention instead of self-attention, the operation becomes as below:
\begin{equation}
\label{eq:CRA}
\begin{aligned}
    & Z_0 =\left[\mathbf{x}^{1}, \mathbf{x}^{2}, \cdots \mathbf{x}^{N}\right]+\mathbf{E}_{\text {pos}} \\
    & Z_{\ell+1}^{\prime} = Z_{\ell} + \operatorname{Cross-Attention}(Z_{\ell}, X_2) \\
    & Z_{\ell+1} = Z_{\ell+1}^{\prime} + \operatorname{FF}(Z_{\ell+1}^{\prime}), ~0 \leq \ell \leq L-1
\end{aligned}
\end{equation}


\subsection{BatchTranslator}

\paragraph{Instance-specific conditioning}

We forget about sequences now. Consider just a data vector $\mathbf{x_1} \in \mathbb{R}^{1 \times d}$ and another data vector $\mathbf{x_2} \in \mathbb{R}^{1 \times d}$. The cross-attention would return $\mathbf{q} = \mathbf{x_1} W_q \in \mathbb{R}^{1 \times d_1}$, $\mathbf{k} = \mathbf{x_2} W_k \in \mathbb{R}^{1 \times d_1}$, $\mathbf{v} = \mathbf{x_2} W_v \in \mathbb{R}^{1 \times d_2}$.
\begin{equation}
\label{eq:attention}
\begin{aligned}
    \operatorname{Cross-Attn}(\mathbf{x_1}, \mathbf{x_2}) & = \operatorname{softmax}\left( \frac{\mathbf{x_1} W_q W_k^T \mathbf{x_2}^T}{\sqrt{d_k}}\right) \mathbf{x_2} W_v \\
    & = \gamma(\mathbf{x_1}, \mathbf{x_2}) \mathbf{x_2}, 
\end{aligned}
\end{equation}
where $\gamma(\mathbf{x_1}, \mathbf{x_2})$ is a nonlinear mixup function that rescales $\mathbf{x_2}$.
Then, the cross-attention transformer layer becomes (especially, the first layer of it):
\begin{equation}
\label{eq:CRA}
\begin{aligned}
    & Z_{1}^{\prime} = \mathbf{x_1} + \gamma(\mathbf{x_1}, \mathbf{x_2}) \mathbf{x_2} \\
    & Z_{1} = Z_{1}^{\prime} + \operatorname{FF}(Z_{1}^{\prime})
\end{aligned}
\end{equation}
which can be viewed as a mixup inside the transformer layer, intuitively.

This, intuitively, gives a super complex non-linear mixup inside the transformer layer, and with the cross-attention mechanism with our associated loss function would act like conditioning $\mathbf{x_1}$ on $\mathbf{x_2}$, to produce a $\mathbf{x_1}$ that is mixed up with $\mathbf{x_2}$, based on $\mathbf{x_1}$'s selection. Intuitively, the product would have the `style' or `essence' of $\mathbf{x_1}$, but the content is changed to $\mathbf{x_2}$.


\paragraph{Label-specific conditioning}

After considering the mixing and translation between individual images or datapoints, we consider conditioning on a group of images with the same label. Specifically, given a batch of data, we consider the latents that share the same label as conditions, and then use it as the K and V into the cross-attention. The produced results are given the label of the shared label. 
Intuitively, this would give a manifold as the conditioning, while in the label space, it still acts like a dirac function of label switching.

Now we consider sequences. Consider a batch of random samples, where $N_{k}$ samples belong to class $k$. When having sample $\mathbf{x_1}$, and we try to mix it with $N_{k}$ samples from class $k$, we would have the below mixing:
% $Q K^{T}$ would give a $N$ by $N$ matrix, where each item at the $i$-th row and $j$-th column would gives $\mathbf{x_i} W_q W_k^T \mathbf{y_j}^T$. Coupling with $V$, we would have each output of the cross attention as:
\begin{equation}
\label{eq:attention}
    \mathbf{x}_{new} = \sum_{j=1}^{N_k} \operatorname{softmax}\left( \frac{\mathbf{x_1} W_q W_k^T \mathbf{x_2^{(j)}}^T}{\sqrt{d_k}}\right) \mathbf{x_2^{(j)}} W_v
\end{equation}
Thus, the transformer becomes:
\begin{equation}
\label{eq:CRA}
\begin{aligned}
    & Z_{1}^{\prime} = \mathbf{x_1} + \mathbf{x}_{new} \\
    & Z_{1} = Z_{1}^{\prime} + \operatorname{FF}(Z_{1}^{\prime})
\end{aligned}
\end{equation}

Correspondingly, as we want to change the new sample to the conditioning, we have the loss function as:
\[
\begin{aligned}
\mathcal{L} & = CE(g(x_1), y_1) + \sum_{j}^{N_k} CE(g(x_2^{(j)}), y_2) \\
& + \frac{1}{k} * \sum_{1}^{k} CE(g(\operatorname{CrossAttn}(x_1, x_2)), y_2)
\end{aligned}
\]
where $\frac{1}{k}$ is a scaling factor, because every sample is translated to all the labels in order to balance the gradient of training.


\paragraph{Batchwise conditioning with label mixture} Having a resulting feature, that acts like a nonlinear mixup of a batch of data $X$ and another batch of data $Y$. We could merge it with the normal classification process as below.

Consider one sample, and a random batch of images (in the high-dimensional image space) $X$ and $Y$. We have a normal backbone network (e.g. ResNet-50) that would produce two batches of latent vectors $L_x$ and $L_y$. Those are put into the cross-attention transformer together, which creates an augmentation, or mixture of things -- let us say -- $L_m = \operatorname{Trans}(L_x, L_y)$. We train the backbone network $f$, the classifier $g$, and the transformer $\operatorname{Trans}$ together, to encourage the translation process:
\[
y_{\operatorname{soft}} = \operatorname{average}_{i \in batch}(y_i)
\]
\[
\begin{aligned}
\mathcal{L} & = CE(g(x_1), y_1) + CE(g(x_2), y_2) \\
& + CE(g(\operatorname{CrossAttn}(x_1, x_2)), y_{\operatorname{soft}})
\end{aligned}
\]
we denote $t$ as the labels, as the character $Y$ is used.

The first two terms are basically just the normal backbone and classifier optimization. The last term is based on the cross-attention operation we performed, where we encourage the translated results to be similar to the latent of the second batch of data $Y$. Thus, it is almost like we are attempting to build a translator of batches.

\subsection{Back translation for cycle consistency}
% \paragraph{Additional back translation for cycle consistency} 
For additional regularization, and also inspired by the back translation process in NLP \cite{} and the cycle consistency loss in visions \cite{}, we perform another round of BatchTranslation, where the loss function is as below:
\[
\begin{aligned}
\mathcal{L} & = CE(g(\operatorname{Trans}(NEW, L_x)), t_x)
\end{aligned}
\]
which finishes up the back translation process.

This process would help maintain the information within the original image/latent during the translation process. The original `style' information is preserved.

To encourage balance inside the training process, the actual implementation contains two different types. The first one is that each image is translated once, the second one specifically is applied in the second "one2many" setting, where each image is translated to each class, and are translated back.

\begin{figure}[t]
\centering
  \includegraphics[width=0.4\textwidth]{images/back_scheme.png}
  \caption{Two different back translation schemes.}
\end{figure}


\subsection{Unifying BatchTranslator and BatchFormer with the perspective of label augmentation}

% BatchTranslator takes a batch of data in the most normal way.

\paragraph{BatchFormer}

BatchFormer is a plug-able component that operates after a normal encoder. Consider a normal encoder $f(x)$ that produces a latent space $l: \mathbb{R}^d$, BatchTranslator operates on top of the latents $l$. A normal $l$ would have a shape of $\mathbb{R}^{B\times d}$, where $B$ is the batch size. BatchTranslator would operate the transformer by considering $B$ as the length of the sequence, by transforming it into a shape of $L_1: \mathbb{R}^{1 \times B\times d}$. The transformer operates on this sequence, and would produce a transformed vector of shape $L_2: \mathbb{R}^{1 \times B\times d}$.
There is going to be a classifier after this to map the latent space into the label space, which we denote as $g(l)$. BatchFormer would have the loss function as below:
\[
\mathcal{L} = CE(g(L), t) + CE(g(\operatorname{SA}(L)), t)
\]

\paragraph{BatchTranslator with permuted batches}

BatchTranslator, normally, would operates on two batches of data $X$ and $Y$. However, consider the following scenario: Having $L$ as the latent representation produced by the above procedure, we consider creating $L_{perm} = L[perm]$, which is a randomly permuted version of $L$. Feeding the resulting $L$ and $ L_{perm}$ into the cross-attention transformer will give exactly the same result as what is being processed by the self-attention transformer, as used in BatchFormer. The only difference between BatchFormer and BatchTranslator is how the label space is formed -- the label space of BatchFormer is always the same as the label that corresponds to $L$; while the label space of BatchTranslator is always a random permutation of the labels that correspond to $L$.

Then how could that be useful at all? The intuition is that, learning the labels of $L$ after self-attention is a trivial process, as the transformer can easily learn an identity matrix out of it. The regularization that is being enforced is really relaxed. However, by performing label permuting, we are encouraging the latent space to really be mixed up, which would give strong latent space augmentation.


\subsection{Understanding what is actually happening through the lens of alignment and uniformity}

I don't really understand the results, so we must develop some way to understand it somehow. Maybe the matrics in \cite{wang2020understanding} would help? At least I can try.

Tested using uniformity matrix on the latents, and they are widely different (between ERM and ERM+BT). It seems like the latent representation produced by BT would shape more like a sphere, without being explicitly regularized to do so.
\[
\begin{aligned}
& \mathcal{L}_{\text {align }}(f ; \alpha) \triangleq \mathbb{E}_{(x, y) \sim p_{\text {pos }}}\left[\|f(x)-f(y)\|_2^\alpha\right] \\
& \mathcal{L}_{\text {uniform }}(f ; t) \triangleq \log \mathbb{E}_{x, y \stackrel{\text { i.i.d. }}{\sim} p_{\text {data }}}\left[e^{-t\|f(x)-f(y)\|_2^2}\right] . \\
&
\end{aligned}
\]
The alignment loss represents how the latents from the same class should be close to each other. The uniform loss represents how the latents should be diverse, thus that they form a unit sphere inside the high-dimensional space. As shown in \cite{wang2020understanding}, they are desired properties in self-supervised learning algorithms when forming the representation, and thus is also desired properties for us.

==> texts/method_Feb8.tex <==
\section{Method}

% \subsection{Background}

\subsection{Overall method}

% According to \cite{bansal2022cold}, diffusion model or diffusion step can be treated as the below noising process and denoising process.

% Warning!!! below text mostly copied from cold diffusion paper
% Warning!!! below text mostly copied from cold diffusion paper
% Warning!!! below text mostly copied from cold diffusion paper
Consider $x_0 \in \mathbb{R}^N$ as a datapoint inside the original dataset.
There is a degradation operator $D$, that is controllable via a human-defined severity parameter $t$, that can create a noisy sample $x_t=D\left(x_0, t\right)$. The output distribution $D\left(x_0, t\right)$ of the degradation should vary continuously in $t$, and in most works it would follow a Gaussian distribution, but actually, it can just be any distribution \cite{bansal2022cold}. 

The generalized diffusion process also needs a restoration operator $R$ that (approximately) inverts $D$. This operator has the property that
$$
R\left(x_t, t\right) \approx x_0 .
$$
In practice (and most of the existing diffusion model works), this operator is 
 the part that needs actual parameter, which is often implemented via a neural network parameterized by $\theta$. The restoration network is trained via the minimization problem
$$
\min _\theta \mathbb{E}_{x \sim \mathcal{X}}\left\|R_\theta(D(x, t), t)-x\right\|,
$$
where $x$ denotes a random image sampled from distribution $\mathcal{X}$ and $\|\cdot\|$ denotes a norm, which is mostly $\ell_1$ or $\ell_2$. We can use the subscript $R_\theta$ to emphasize the dependence of $R$ on $\theta$ during training.

In the real diffusion models, the diffusion process needs to be performed sequentially, because when having a large $t$, the restoration network $R_\theta$ loses its power. There are many ways to address it via designing new scheduler, but still, the most state-of-the-art diffusion model still would need many steps (iterations) to generate high-resolution images.

%\begin{algorithm}
%\caption{{\bf Ours}}
%\begin{algorithmic}
%    \Statex {\bf Input:} Backbone $f(\cdot)$, classifier $g(\cdot)$, and entropy-regularization parameter $\varepsilon$.
%\Statex{\bf Output:} Dictionaries $\cal{D}$, coefficients $\cal{A}$, align plans $\{\mathbf{P}_{i,\l}\}_{i,\l}$.
%\State{ Initialize:}~$\mathbf{P}_{i\l},~D_{\l},~\alpha_{i\l}$, $\forall$ $i,\l$.
%\While{not converging}
%\State $\{\mathbf{P}_{i\l}\}\leftarrow$\url{UpdateTransport}(${\cal{D}}$, %${\cal{A}}$)
%\State ${\cal{A}}\leftarrow$\url{UpdateClassify}($\{\mathbf{P}_{i,l}\}$,$\cal{D}$)
%\State ${\cal{D}}\leftarrow$\url{UpdateStructure}($\{\mathbf{P}_{i,l}\}$, $\cal{A}$)
%\EndWhile
%\end{algorithmic}
%\end{algorithm}

\begin{algorithm}[h]
\SetAlgoLined
    % \PyComment{going to have indentation} \\
    \PyCode{def train(l, y, ft, bt):} \\
    \Indp   % start indent
        \PyComment{l: latent} \\
        \PyComment{y: label} \\
        \PyCode{l$_f$ = ft(l)} \\ % \PyComment{inline comment} \\ 
        \PyCode{l$_b$ = bt(l$_f$, l)} \\
        \PyCode{y$_{soft}$ = average(y)} \\
        \PyCode{loss1 = criteria(l, y)} \\
        \PyCode{loss2 = criteria(l$_f$, y$_{soft}$)} \\
        \PyCode{loss3 = criteria(l$_b$, y)} \\
        \PyCode{return loss1 + loss2 + loss3} \\       
    \Indm % end indent, must end with this, else all the below text will be indented
%    \PyComment{this is a comment} \\
%    \PyCode{your code}
\caption{PyTorch-style pseudocode}
\label{algo:your-algo}
\end{algorithm}


\subsection{Generalized transformer}

\paragraph{Self-attention}
% \subsection{Transformer basics}

% please remember to edit text, copied from EIT
Transformers consider sequences of data in the format of $X = [\mathbf{x}^{1}\ \mathbf{x}^{2}\ \dots \  \mathbf{x}^{N}]^T \in \mathbb{R}^{N \times d}$ consisting of $N$ tokens of $d$-dimensions.
The self-attention mechanism derives queries $Q$, keys $K$, and values $V$ by performing linear projections for each token embedding, which gives $Q = XW_Q, K = X W_K , V = X W_V $, where $Q \in \mathbb{R}^{N \times d_q}$, $K \in \mathbb{R}^{N \times d_k}$, $V \in \mathbb{R}^{N \times d_v}$. The self-attention gives:
\begin{equation}
\label{eq:attention}
    \operatorname{Attention}(Q,K,V) = \operatorname{softmax}\left( \frac{1}{\sqrt{d_k}}{Q K^{T}}\right) V,
\end{equation}
where $\operatorname{softmax}(\cdot)$ gives row-wise softmax normalization.

\paragraph{Cross-attention}

Cross-attention is basically the same, it is just that you need to change $Q = X_1W_Q, K = X_2 W_K , V = X_2 W_V $ for a pair of data $X_1$ and $X_2$.


\paragraph{Transformer}

% please remember to edit text, copied from EIT
The transformer architecture as a model building block consists of many ($L$) layers of the below operations:
\begin{equation}
\label{eq:MSA}
\begin{aligned}
    & Z_0 =\left[\mathbf{x}^{1}, \mathbf{x}^{2}, \cdots \mathbf{x}^{N}\right]+\mathbf{E}_{\text {pos}} \\
    & Z_{\ell+1}^{\prime} = Z_{\ell} + \operatorname{Attention}(Z_{\ell}) \\
    & Z_{\ell+1} = Z_{\ell+1}^{\prime} + \operatorname{FF}(Z_{\ell+1}^{\prime}), ~0 \leq \ell \leq L-1
\end{aligned}
\end{equation}
where $Z_0$, as the initialization, sums up the individual token embedding and their positional embedding $\mathbf{E}_{\text {pos}}$ (which is optional, and not used in our architecture). Each transformer layer is the combination of the Attention operation ($\operatorname{Attention}(\cdot)$), the nonlinear projection ($\operatorname{FF}(\cdot)$, stands for feedforward network or MLP), and residual connections.

When feeding the network pairs of data points $X_1$ and $X_2$, and using cross-attention instead of self-attention, the operation becomes as below:
\begin{equation}
\label{eq:CRA}
\begin{aligned}
    & Z_0 =\left[\mathbf{x}^{1}, \mathbf{x}^{2}, \cdots \mathbf{x}^{N}\right]+\mathbf{E}_{\text {pos}} \\
    & Z_{\ell+1}^{\prime} = Z_{\ell} + \operatorname{Cross-Attention}(Z_{\ell}, X_2) \\
    & Z_{\ell+1} = Z_{\ell+1}^{\prime} + \operatorname{FF}(Z_{\ell+1}^{\prime}), ~0 \leq \ell \leq L-1
\end{aligned}
\end{equation}

\paragraph{MetaTransformer}

Recently, \cite{yu2022metaformer} shows that the whole cross-attention and self-attention thing isn't necessary for images. Specifically, the self-attention operation can be replaced by pooling operation, which requires no parameters at all, below is their formulation:
\begin{equation}
\label{eq:MSA}
\begin{aligned}
    & Z_0 =\left[\mathbf{x}^{1}, \mathbf{x}^{2}, \cdots \mathbf{x}^{N}\right]+\mathbf{E}_{\text {pos}} \\
    & Z_{\ell+1}^{\prime} = Z_{\ell} + \operatorname{Mixing}(Z_{\ell}) \\
    & Z_{\ell+1} = Z_{\ell+1}^{\prime} + \operatorname{FF}(Z_{\ell+1}^{\prime}), ~0 \leq \ell \leq L-1
\end{aligned}
\end{equation}
where $\operatorname{Mixing}$ can be any mixing operation, which can be a simpler spatial MLP, or even a parameter-less operation as the Pooling operation.


\subsection{Our method}

\paragraph{In general}

Consider a random batch of data $X$ that is associated with label $Y$, a normal backbone encoder $f(\cdot)$, a classifier $g(\cdot)$. For a normal training process with ERM loss function, we have:
\[
\mathcal{L} = \mathbb{E}[\operatorname{CE}(g(f(X)), Y) ]
\]
Our model follow the same process during inference, however, during training, we have a new $D(\cdot)$ as the noising operator, and $R(\cdot)$ as the restoration operator. We have $X_{\operatorname{noise}} = D(X)$, and $X_{\operatorname{r}} = R(D(X))$, and thus, the general concept becomes:
\[
\begin{aligned}
\mathcal{L} & = \mathbb{E}[\operatorname{CE}(g(f(X)), Y) ] \\
& + \mathbb{E}[\operatorname{Align}(D(f(X)), \operatorname{noise}) ] \\
& + \mathbb{E}[\operatorname{Align}(R(D(f(X))), Y) ]
\end{aligned}
\]


\paragraph{Classifier-guided diffusion}

Our `diffusion' step is not a real diffusion step, instead, we use the classifier $g(\cdot)$ and ERM loss function as the regularization.
Thus, the final loss function is:
\[
\begin{aligned}
\mathcal{L} & = \mathbb{E}[\operatorname{CE}(g(f(X)), Y) ] \\
& + \mathbb{E}[\operatorname{CE}(g(D(f(X))), Y_{\operatorname{noise}}) ] \\
& + \mathbb{E}[\operatorname{CE}(g(R(D(f(X)))), Y) ]
\end{aligned}
\]
where $Y_{\operatorname{noise}}$ is the mixture of labels:
\[
Y_{\operatorname{noise}} = \operatorname{average}(Y)
\]

\paragraph{Generating noisy sample and recovering them with sample-to-sample relationship transformer}

The question is: how to create a good $D(\cdot)$ and $R(\cdot)$? Inspired by BatchFormer and StableDiffusion, we used cross-attention transformers that aim to degrade the latents to confuse the classifier.

Specifically, we tested the self-attention/cross-attention transformer, as well as the poolformer/cross-attention transformer. Specifically, when considering only two individual samples $\mathbf{x_1}$, $\mathbf{x_2}$, we would have:
\begin{equation}
\label{eq:attention}
\begin{aligned}
    \operatorname{Cross-Attn}(\mathbf{x_1}, \mathbf{x_2}) & = \operatorname{softmax}\left( \frac{\mathbf{x_1} W_q W_k^T \mathbf{x_2}^T}{\sqrt{d_k}}\right) \mathbf{x_2} W_v \\
    & = \gamma(\mathbf{x_1}, \mathbf{x_2}) \mathbf{x_2}, 
\end{aligned}
\end{equation}
thus, when having a batch of data, we would have:
\begin{equation}
\label{eq:attention}
\begin{aligned}
    \operatorname{Cross-Attn}({X_1}, {X_2}) = \sum_{x_2 \in X_2} \gamma({X_1}, \mathbf{x_2}) \mathbf{x_2}, 
\end{aligned}
\end{equation}
which basically would create something noise, but is close enough to the original data.

When recovering, the same operation can be used again, while the aim of the second operation is to use $X_1$ to find the `consistent' information inside $X_2$. The different functionality is regularized by the loss function.



\subsection{Understanding the method}
% \paragraph{Additional back translation for cycle consistency} 
\paragraph{From the perspective of cycle consistency}
For additional regularization, and also inspired by the back translation process in NLP \cite{} and the cycle consistency loss in visions \cite{}, we perform another round of BatchTranslation, where the loss function is as below:
\[
\begin{aligned}
\mathcal{L} & = CE(g(\operatorname{Trans}(NEW, L_x)), t_x)
\end{aligned}
\]
which finishes up the back translation process.

This process would help maintain the information within the original image/latent during the translation process. The original `style' information is preserved.

To encourage balance inside the training process, the actual implementation contains two different types. The first one is that each image is translated once, the second one specifically is applied in the second "one2many" setting, where each image is translated to each class, and are translated back.

\paragraph{From the perspective of sample-to-sample relationship}

Text.


\subsection{Evaluate the latent space through the lens of alignment and uniformity}

I don't really understand the results, so we must develop some way to understand it somehow. Maybe the matrics in \cite{wang2020understanding} would help? At least I can try.

Tested using uniformity matrix on the latents, and they are widely different (between ERM and ERM+BT). It seems like the latent representation produced by BT would shape more like a sphere, without being explicitly regularized to do so.
\[
\begin{aligned}
& \mathcal{L}_{\text {align }}(f ; \alpha) \triangleq \mathbb{E}_{(x, y) \sim p_{\text {pos }}}\left[\|f(x)-f(y)\|_2^\alpha\right] \\
& \mathcal{L}_{\text {uniform }}(f ; t) \triangleq \log \mathbb{E}_{x, y \stackrel{\text { i.i.d. }}{\sim} p_{\text {data }}}\left[e^{-t\|f(x)-f(y)\|_2^2}\right] . \\
&
\end{aligned}
\]
The alignment loss represents how the latents from the same class should be close to each other. The uniform loss represents how the latents should be diverse, thus that they form a unit sphere inside the high-dimensional space. As shown in \cite{wang2020understanding}, they are desired properties in self-supervised learning algorithms when forming the representation, and thus is also desired properties for us.








%%%%%%%%%%%%%%%%% OLD INTRO SECTION


% Corrupting data is a key part of many approaches in modern ML - for augmenting data, blah, and more recently for diffusion models
% here, we explore whether the process of corrupting and restoring data can be a useful latent augmentation for improving learning
% we show this works in many contexts and in diverse datasets



%The essence of many state-of-the-art machine learning algorithms is based on the corruption and the restoration of the original data. 
% The beginning of self-supervised learning is based on the development of Noise Contrastive Estimation (NCE) loss \cite{gutmann2010noise,ma2018noise} (it is actually also related to GANs \cite{goodfellow2020generative}). 
%Masked autoencoder is based on masking the majority of the data and recovering them.
%More recently, diffusion models showed that by adding noise into the image in either a deterministic way \cite{bansal2022cold,daras2022soft} or a continuous way can also achieve state-of-the-art performance in image synthesis. 
% Below is more loosely related and hard to argue. But I found the connection between NCE and negative sampling interesting.
% Moreover, even self-supervised learning algorithms (e.g. SimCLR and MoCo) are based on strong data augmentation that tends to distort the image while maintaining its semantic information, and the Noise Contrastive Estimation (NCE) loss \cite{gutmann2010noise,ma2018noise} they used is closely related to negative sampling.

%\colortext{Would the below logic be better?}
% Human visual system is robust to the corruption of data, as it naturally recovers the semantic meaning of the image. This special ability of the human visual system lets us easily generalize across domains. This property, however, is lacking in deep learning networks. Most of the networks only work well when the training data and testing data follow the i.i.d. assumption, and when there do exist domain shifting, the performance would suffer greatly.


% Recently, there has been a lot of works that aims to explore how the process of data corruption and data restoration can be effectively used to learn a better representation of the image. There are algorithms like Masked autoencoders and diffusion models. However, they focus on training on diverse set of training data. In this work, instead, we explore how the process of corruption and restoration can be directly applied on latent space, and can be used to help the network to be robust against the domain shifting issue.

% The collection of large-scale training data samples has enabled a lot of great success in various domains \cite{radford2021learning,rombach2022high}. However, in a real-world setting, the collection of large-scale labeled datasets can be challenging, and the collection source would result in a lot of domain shifting. To address this issue, researchers have been exploring solutions from several frontiers. There are data augmentation works and latent augmentation works. However, it is still challenging to find good general-purpose solution to this issue.

%1. Diffusion models (DMs) are achieving state-of-the-art performance in terms of image synthesis, outperforming more traditional GAN, and it became popular because of that.
%2. Aside from only image synthesis, it has many applications. In terms of single-modality application, there is conditional (on another image) image synthesis, super-resolution, and impainting. In terms of multimodal applications, there is language-guided image synthesis.
%3. Diffusion models are essentially denoising autoencoders, that are guided by a sequential generative process (need to check more accurate terminology). Different from GAN, which is mathematically equivalent to finding a saddle point in the optimization space, DMs are built based on likelihood, thus, they have great advantage preventing mode-collapse and they are really stable to train.
% 4. However, the disadvantage is that (1) They do require a decent amount of parameters, mostly because they are used for image synthesis. It would be great if researchers can explore a way to not use so many parameters at all. (2) The inference time requires a decent amount of iterations, because the whole thing works like a Markov chain. Although there are many schedulers \cite{DDIM} to replace \cite{DDPM} that attempts to accelerate the steps in middle, it still takes a lot of inference time, which limit the potential of using DMs in more applications, such as as an assistance model during the training of another model.

%\begin{figure}[t]
%\centering
%  \includegraphics[width=0.45\textwidth]{images/overview_dg_pool.png}
%  \caption{Overview of the high-level idea of the model. We can either use a real latent space figure, or a toy figure like this.}
%\end{figure}

% To fill this gap, in this paper, we explore the usage of the most essential part of DMs, the noising and denoising part, as data augmentation operations. 
% \colortext{Okay, guess we need to introduce how DM works at the very beginning.}
% 1. Our approach basically adds noise into the latent space to create noisy samples, and then perform latent restoration during training.
% 2. To make this approach really work, we majorly rely on two things: (1) we used transformer to create new latent points that are supposed to be noisy, and restore it with another transformer. (2) We used sample-to-sample relationship to generate new latent points, so that they are just noisy enough to not be distinguished by classifier, but is distinguishable, or recoverable by a cross-attention transformer. (3) We used classifier-guided diffusion step, which gives a Cross-Entropy loss function instead of a pixel-wise loss function like the L1 or L2 loss that is commonly used in DMs, and that gives us both flexibility and additional training (thus robustness) of the classifier. 
% 3. With all those things combined, we designed a flexible thing during training, that is completely removable during testing, that can be viewed as a robust data augmentation operation. 
% \colortext{If you are using another model, does that still count as data augmentation?}


% We apply the method on a variety of tasks, including (1) a toy application on medical image classification on a set of 2D and 3D tasks. (2) complete and systematic application on domain generalization task on standard benchmarks (3) comparison with BatchFormer \cite{hou2022batchformer} on long-tail recognition tasks. To quantify the improvements, and to further understand why the proposed method is effective, we used uniformity and alignment to understand the latent quality. Our model provides a very good exploration along this direction, in terms of discovering how much DMs, or the principle of DMs, can be used in a normal classification training process, or other wise range of tasks.


% for a variety of task that are within the low-data or domain shifting range of applications.
% Recently, BatchFormer \cite{hou2022batchformer} demonstrated that using a transformer to learn relationships inside mini-batches can be successful. This demonstrated the potential of using sample-to-sample relationship in a non-linear way can be really useful and improve the learning of representations. However, because of the approach kind of encourage learning an identity matrix, its performance isn't as good as what it should be. % hmm how to say this ??

% It is a critical problem to learn a representation that is invariant to individual variances.


% Different from domain adaptation (DA), which has access to the unlabelled samples from the testing domain during the training stage, domain generalization (DG) does not  access the target domain at all during training. 
% good opening 
% HETEROGENEOUS DOMAIN GENERALIZATION VIA DOMAIN MIXUP

% To address the problem of domain shifting using the sample-to-sample relationship, we explored the content/style mixing \cite{zhou2021domain}, and developed a translation approach. Specifically, we used the cross attention that is used in \cite{jaegle2021perceiver,rombach2022high}, we translate one sample to another sample, and use the mixture of latent with cross attention to guide the learning. Different from BatchFormer \cite{hou2022batchformer}, we encourage the cross-attention, so that the resulting latent space is very different from an identity matrix, but more like a mixture of styles.

%To conclude, our work has the below contributions: 
% (1) We explored the possibility to use the process of diffusion and latent restoration as an effective data augmentation operation on images, assisting a normal backbone model (e.g. ResNet-50). This is the first work that conceptually do this 
% \colortext{Need to check if this claim is accurate};
% (2) We combine the sample-to-sample relationship research with a classifier-guided diffusion process, which created a pluggable and removable part of the model, that is parameter-free during inference;
% (3) We demonstrated the robustness of our method on domain generalization tasks, which opened up a lot of possibilities for the proposed method;
% (4) We applied a set of visualization and metrics to understand the method.

==> texts/method_eva.tex <==
\section{Method}

% \subsection{Background}


\subsection{Our method}

Inspired by diffusion models \cite{rombach2022high}, our data augmentation operation is learned through a {\em degradation} step and {\em restoration} step. 
% The learning of the degradation and restoration operators work hand in hand at the batch level. 
%Critically, after augmenting samples in the batch, we use cross-attention to query the sample using its relative position in the original latent distribution, using keys from the original latents to learn a back translation with queries from the augmented latents. 
We visualize the forward and backward steps in our process and overview of architecture in Figure 2 and provide pseudocode in Algorithm~\ref{algo:main}.
%Our algorithm is built based on both the batch-wise nonconvex mixture of samples to perform latent degradation, as well as the classifier-guided latent restoration. 
The method can be implemented easily and fit into the mini-batch training process and can be removed during inference. 

\begin{algorithm}[h]
\label{code:alg}
\SetAlgoLined
    % \PyComment{going to have indentation} \\
    \PyCode{def train(z, y, g, ft, bt):} \\
    \Indp   % start indent
        % \PyComment{l: latent} \\
        % \PyComment{y: label} \\
        \PyCode{z$_f$ = ft(z)} \\ % \PyComment{inline comment} \\ 
        \PyCode{z$_b$ = bt(z$_f$, z)} \\
        \PyCode{y$_{soft}$ = average(y)} \\
        \PyCode{loss1 = criteria(g(z), y)} \\
        \PyCode{loss2 = criteria(g(z$_f$), y$_{soft}$)} \\
        \PyCode{loss3 = criteria(g(z$_b$), y)} \\
        \PyCode{loss = loss1 + loss2 + loss3} \\   
        \PyCode{loss.backward()} \\
    \Indm % end indent, must end with this, else all the below text will be indented
%    \PyComment{this is a comment} \\
%    \PyCode{your code}
\caption{Batch Translator Pseudocode}
\label{algo:main}
\end{algorithm}


\subsubsection{High-level Objective}~ 
Consider $(x, y)$ as an original datapoint and label pair from our data distribution $(\mathcal{X}, \mathcal{Y})$. Let $z = f(x)$ denotes the embedding of $x$ after the encoder $f$.
% and $Z \in \mathbb{R}^{L \times B}$ contains the representations of a batch of samples from the dataset, where $L$ is the dimension of the latent space and $B$ is the size of the batch. 
The overall objective of the method is to learn a latent degradation operator $D_{\mu}$ that produces embeddings that would `confuse' the prediction of the labels; and a latent restoration operator $R_{\theta}$ that would `denoise' the prediction of the labels.
% denote the forward step to augment latents and let $R_{\theta}$ denote the reverse mapping that (approximately) inverts $D$ to produce a batch that is mapped back to their corresponding and correct labels. 
% In this work, we consider a supervised setting where we have labels $y$ and an appropriate loss function $\ell(\cdot, \cdot)$ that matches the prediction problem at hand (for instance, cross entropy). 
This high-level objective can be specified as:
%\[
%\min _{f, g, \theta, \mu} \mathbb{E}_{x \sim \mathcal{X}} ~ \ell(g(z), y) +  \ell(g(R_\theta(D_{\mu}(z)), y)
%\]
\[
\begin{aligned}
z \Rightarrow y \\
D_{\mu}(z) \nRightarrow y \\
R_\theta(D_{\mu}(z)) \Rightarrow y
% \ell(g(z), y) \neq \ell(g(D_{\mu}(z)), y), \\
% \ell(g(z), y) \approx \ell(g(R_\theta(D_{\mu}(z)), y),
\end{aligned}
\]
where $g$ is a classifier that is trained to predict the output labels $y$, and $D_{\mu}(z)$ introduces some non-trivial perturbation to the latent variables. Thus, our goal is to learn a degradation and restoration operator to return the latents back to their original distribution of labels, but this doesn't mean that our recovered latent $z_{rec} = R_{\theta}(D_{\mu}(z))$ is close to its original position. In general, without appropriate constraints on the degradation, a trivial solution can be the identity, however, we will next describe a procedure to push the latents away from their original positions to ensure that this doesn't happen.

\subsubsection{Latent degradation with mixtures and soft labels}

In order to encourage the datapoints from different domains to mix with each other and provide additional sample information during training, we create latent mixtures and soft labels to guide them in the degradation step.
For each latent, we augment it through the following spatial pooling operation:
\[
\widetilde{z} \sim D( \widetilde{z} \mid z) = z + \operatorname{Pooling}(\operatorname{Subset}(Z)),
\]
where the pooling operator augments $z$ by adding a mixture of other latent samples in the same batch to get an augmented sample $\widetilde{z}$. In practice, we implement this pooling operation with Layerwise normalization and an MLP, inspired by the design of PoolFormer \cite{yu2022metaformer}. We also implemented a variant with the normal self-attention transformer with dropout (see Appendix XX). 
%During training, we generate a corrupted sample $z_{d}$ with a random subset of samples from the batch. 

In order to encourage this forward procedure to map the data to a common distribution that may encourage mixing of samples across different domains, 
we regularize the degraded samples to be aligned with soft or noisy labels $y_{soft}$. We can write out the loss associated with our forward operation as:
%\[
%\mathcal{L} =  \underbrace{\ell(g(z), y)}_{\text{original}} + \underbrace{ \ell(g(R_\theta(D_{\mu}(z)), y)}_{\text{restore}} + \underbrace{\ell(g(D_{\mu}(x), y_{\operatorname{soft}})}_{\text{corrupt}}
%\]
\[
\mathcal{L}_{\text{degrade}} = \ell(g(D_{\mu}(z), y_{\operatorname{soft}})
\]
In practice, we set  $y_{soft} = \operatorname{average}(Y_b)$ to the average over all the one-hot labels in the batch. However, we also test other label distributions in XX.

%As our batch size is large enough to cover the classes, for a balanced dataset we will obtain a nearly uniform distribution for our soft label as our target distribution. 
%We provide an intuitive explanation in Appendix. 


% implement this forward operation with a very lightweight model called Poolformer. [Explain Poolformer in more detail here]

%In practice, we found that setting the soft labels to the empirical mean for the batch works well in practice. In this case, the soft labels for each batch would be given by:
% $y_{\operatorname{soft}} = \frac{1}{B} \sum_{y_i \in Y_b} y_i.$ We provide results for other variants in Section (X).

% We implement this forward operation with a very lightweight model called Poolformer. [Explain Poolformer in more detail here]


\subsubsection{Classifier-guided restoration with cross-attention}~

Both the degradation  and restoration operators work together in tandem to ensure that the latents can be recovered. In other words, while performing latent degradation, we would like $z_{d}$ to still be distinguishable, or recoverable, such that it still contains the trace of the original $z$ and we can recover its class.

To restore the latents back to their original classes, our model leverages a cross-attention mechanism that  computes  queries $Q$ from the corrupted latents $\widetilde{Z}$ and the keys $K$ and values $V$  from the original latents $Z$:
%\[
%Q = Z_B W_Q, K = Z_{corr} W_K , V = Z_{corr} W_V
%\]
\[
Q = \widetilde{Z} W_Q, K = Z W_K , V = Z W_V
\]
As the attention mechanism is permutation-invariant, the ordering of the output would be decided based on the ordering of the queries, which enforces the the corrupted latents to contain the information that is enough to recover the class of the original latents. At the same time, $Z$ serves as a  knowledge bank. 
% The intuition behind this is XX and YY.
Thus, intuitively, the restoration operator is learning to invert the augmentations based on cross-attention:
\[
R(z_{r} \mid z_{d}) = \operatorname{softmax}(QK^T) V,
\]
where the corrupted latents select  similar samples from the original latents. In contrast to an autoencoder or reconstruction loss, we use classifier guidance instead of a $\ell_1$ or $\ell_2$ loss on the latents to regularize the reverse process. This relaxed regularization process aims to encourage samples from different domains to be mapped to their corresponding class during restoration, thus creating a type of domain-invariance and more robustness in the classification task.


\subsubsection{Combined losses}

Thus overall our method aims to optimize a combination of the following three losses:
\[
\mathcal{L} =  \underbrace{\ell(g(z), y)}_{\text{original}} + \underbrace{ \ell(g(R_\theta(D_{\mu}(z)), y)}_{\text{restore}} + \underbrace{\ell(g(D_{\mu}(x), y_{\operatorname{soft}})}_{\text{degrade}}
\]
As you can see, we use the classifier to both guide the corrupted latents towards misclassification and back to their correct labels after restoration. Additionally, a key property of our objective is the use of samples within out batch to both create augmentations and also as a way to restore the batch, by using sample-to-sample relationships.

% \subsection{Discussion of method and comparisons}
% Mixup was using the below distribution created by convex optimization:
% \[
% \begin{aligned}
% &\mu\left(\tilde{x}, \tilde{y} \mid x_i, y_i\right) = \\
% &\frac{1}{n} \sum_j^n \underset{\lambda}{\mathbb{E}}\left[\delta\left(\tilde{x}=\lambda x_i+(1-\lambda) x_j, \tilde{y}=\lambda y_i+(1-\lambda) y_j\right)\right]
% \end{aligned}
% \]
% our formulation, instead, consider the mini-batch distribution directly with the alternative distribution:
% \[
% \begin{aligned}
% &\mu\left(\tilde{x}, \tilde{y} \mid x_i, y_i\right) = \\
% &\frac{1}{n} \sum_j^n \underset{\lambda}{\mathbb{E}}\left[\delta\left(\tilde{x}=D_\theta (x_i \mid X_b), \tilde{y} = \operatorname{average}(Y_b) \right)\right]
% \end{aligned}
% \]
% which creates a non-convex combination of samples following the distribution $\mu(\tilde{x}, \tilde{y})$. This distribution is later used in the restoration operator to generate a diverse set of $x^{\operatorname{recover}}$.




%From the perspective of content style separation, the queries provide the content, while the condition provides the style.


%Putting this together, we have the following loss:
%\[
%\min_{g, f, \theta, \mu}  g( z, y) + g( R_{\theta}\left( D_{\mu} ( z , Z_B ) , \widetilde{Z_B} \right), y), 
%\]



%In most of the traditional works, the degradation operator and the restoration operator are trained by the below minimization problem that operates directly on the data space:
%\[
%\min _{\theta, \mu} \mathbb{E}_{x \sim \mathcal{X}}\left\|R_\theta(D_{\mu}(x))-x\right\|,
%\]
%where $x$ denotes a random image sampled from the data distribution $\mathcal{X}$ and $\|\cdot\|$ denotes a norm, which is mostly $\ell_1$ or $\ell_2$. % We can use the subscript $R_\theta$ to emphasize the dependence of $R$ on $\theta$ during training.

% In the real diffusion models, the diffusion process needs to be performed sequentially, because when having a large $t$, the restoration network $R_\theta$ loses its power. There are many ways to address it via designing new scheduler, but still, the most state-of-the-art diffusion model still would need many steps (iterations) to generate high-resolution images.


%In what we have described until now, we use the 

%We use the classifier $g(\cdot)$ and loss function $\ell(\cdot, \cdot)$ to perform guidance, to optimize the below function:
%\[
%\min _{\theta, \mu} \mathbb{E}_{x \sim \mathcal{X}} \ell(g(x), y) + \mathbb{E}_{x \sim \mathcal{X}} \ell(g(R_\theta(D_{\mu}(x)), y)
%\]
%Thus, the restoration is relaxed, such that the restoration is regularized such that it will return to the original distribution of labels instead of the original distribution of itself.

%he second term is to minimize the below risk:
%\[
%R = \int \ell(g(x), y) \mathrm{d} P(x^{\operatorname{recover}}, y)
%\]
% where $\left(x_{i}^{\operatorname{recover}}, y_i\right) \sim P$ is a more diverse set of samples than the distribution of the original data $\left(x_{i}, y_i\right) \sim P$.
% \textit{Remark. Consider the domain generalization setting, where the same label $y$ could map to $x_1$ and $x_2$ from two different distributions, this classifier-guided (soft) process of latent restoration might allow the restoration of $x_1$ to $x_2$.}
%\paragraph{Building soft-label for degraded samples}
%In order to make sure that $\left(z_{i}^{\operatorname{rec}}, y_i\right) \sim P$ provides a more diverse set of samples, we need to first ensure the degradation provides a diverse set of samples. 



%\subsection{Understanding the method through the lens of content/style separation of classifier}
% \paragraph{Additional back translation for cycle consistency} 

% We provide an intuitive explanation of the method from the perspective of content/style separation of the latent space. Intuitively, for the domain generalization perspective, each sample from the dataset should contain three parts of information: (1) The class-related property, which is one specific type of mutual information, that is learned by minimizing the loss of classifier. (2) The domain-related property, which is the `style', a classifier that should be ignored by the classifier, but in the domain generalization setting there are few `styles' that are obvious to the learning process. (3) Instance-specific variance.




\subsection{Assessing representation quality with alignment and uniformity metrics}

To further understand how the proposed method would encourage the latent representation to help in terms of generalization (robust to domain shifting) and classification (clustering of the same class), we used the latent representation evaluation methods proposed in \cite{wang2020understanding}.
Specifically, the latent representation can be evaluated through the lens of alignment and uniformity. Alignment measures the `closeness' of features from the same class; while uniformity measures the distribution of the (normalized) features on
the hypersphere, which can be understood as the diversity and spread of samples throughout the space. 

The aligmment of the learned  representations is measured as:
\begin{equation}
\mathcal{L}_{\text {align }}(f ; \alpha) \triangleq \mathbb{E}_{(x_1, x_2) \sim p_{\text {pos }}}\left[\|f(x_1)-f(x_2)\|_2^\alpha\right],
\end{equation}
where $(x_1, x_2) \sim p_{\text {pos}}$ draws samples from the same class, and $\alpha$ is a hyperparameter.

The uniformity of the representations is defined as:
\begin{equation}
\mathcal{L}_{\text {uniform }}(f ; t) \triangleq \log \mathbb{E}_{x_1, x_2 \stackrel{\text { i.i.d. }}{\sim} p_{\text {data }}}\left[e^{-t\|f(x_1)-f(x_2)\|_2^2}\right],
\end{equation}
where in this case the samples $(x_1, x_2)$ are across the entire dataset and $t$ sets the bandwidth of our radial basis function used to measure distance.

As shown in \cite{wang2020understanding}, those two properties are desired properties in representation learning. 
To extend the use of the metrics, and to further understand how the representation in domain generalization settings can be evaluated beyond classification accuracy, we compare our methods with other methods based on those metrics.
